Dynamic Resource Allocation in the Cloud with Near-Optimal Efficiency

Cloud computing has motivated renewed interest in resource allocation problems with new consumption models. A common goal is to share a resource, such as CPU or I/O bandwidth, among distinct users with different demand patterns as well as different quality of service requirements. To ensure these service requirements, cloud offerings often come with a service level agreement (SLA) between the provider and the users. An SLA specifies the amount of a resource a user is entitled to utilize. In many cloud settings, providers would like to operate resources at high utilization while simultaneously respecting individual SLAs. There is typically a tradeoff between these two objectives; for example, utilization can be increased by shifting away resources from idle users to "scavenger" workload, but with the risk of the former then becoming active again. We study this fundamental tradeoff by formulating a resource allocation model that captures basic properties of cloud computing systems, including SLAs, highly limited feedback about the state of the system, and variable and unpredictable input sequences. Our main result is a simple and practical algorithm that achieves near-optimal performance on the above two objectives. First, we guarantee nearly optimal utilization of the resource even if compared to the omniscient offline dynamic optimum. Second, we simultaneously satisfy all individual SLAs up to a small error. The main algorithmic tool is a multiplicative weight update algorithm, and a primal-dual argument to obtain its guarantees. We also provide numerical validation on real data to demonstrate the performance of our algorithm in practical applications.

==> version arxiv/Acknowledgments.tex <==
\section*{Acknowledgments}

The authors' work was partially supported by the U.S.\ National Science Foundation via grants CMMI 1552479, AF 1910423 and AF 1717947. We thank Vivek Narasayya for useful discussions.

==> version arxiv/Algorithm.tex <==

\section{Algorithm}\label{sec:algorithm}

%Before we describe the algorithm, we begin with a few preliminaries.

\subsection{Preliminaries}\label{sec:prelim}

For $N\geq 1$, we identify the set of \emph{users} with the set $[N]=\{1, \ldots, N \}$. For $0< \varepsilon< 1$, we call an allocation $\h =(h(1),\ldots, h(N) )\in [0,1]^N$ a \emph{$(1-\varepsilon)$-allocation} if $\sum_i h(i)\leq 1-\varepsilon$. We assume $N\geq 2$, that is, the system consists of at least two users.

For any $t$, we define the set of \emph{active users} at that time as the set of users with non-empty queue, and denote this set by $A_t$. Observe that $h_t(i) = w_t(i)$ for all active users. Let $B_t=[N]\setminus A_t$ be the sets of users with empty queues at time $t$; we call these users  \emph{inactive}. $A_t$ and $B_t$ correspond to the feedback given to the decision maker. Also, let $A_t^1 = \{ i\in A_t : h_t(i)< \beta(i)  \}$ be the set of active users with allocation below their SLA and $A_t^2 = A_t\setminus A_t^1$ be the set of active users receiving at least their SLAs.

We assume without loss of generality that the allocations set by the decision maker always add up to $1$. We propose an algorithm that uses a multiplicative weight strategy to boost a subset of users by multiplying their allocation by factor greater than one. Because the allocations do not sum to one after applying the update, we then project them onto the simplex using the KL-divergence metric. Furthermore, to ensure no user gets an allocation arbitrarily close to zero, we in fact project onto the \emph{truncated simplex},
\[
\Delta_\varepsilon = \{ \x =(x(1),\ldots,x(N)) :  \|\x\|_1 = 1, x(i)\geq \varepsilon/N, \forall i  \}.
\]
To fix notation, let $\pi_{\Delta_\varepsilon}(\cdot)$ be the \emph{projection function} onto $\Delta_\varepsilon$ using Kullback–Leibler divergence (KL-divergence for short), i.e., $\pi_{\Delta_\varepsilon}(\y) := \argmin_{\x \in \Delta_\varepsilon} \sum_i x(i)\log ( x(i) / y(i) )$, where $\y=(y(1),\ldots,y(N) )\in \R_{\geq 0}^N$. In Appendix \ref{sec:projection}, we show how to efficiently compute this projection. The following proposition states some basic facts that are useful in our analysis. The proof appears in Appendix \ref{sec:projection}.
%
\begin{proposition}\label{prop:projection}
	Let $\y \in \R_+^N$, $\x =\pi_{\Delta_\varepsilon}(\y)$, and $S=\{ i : x(i) = \frac{\varepsilon}{N}  \}$. Then:
	\begin{enumerate}[label=(\alph*)]
		\item If $y(1)\leq y(2)\leq \cdots \leq y(N)$, then $S=\{1,\ldots, k  \}$ for some $k\geq 0$.
		
		\item $x(i) = y(i) e^{\mu_i} C$, where   $ C= \left( \frac{1-\frac{\varepsilon}{N}|S|}{\sum_{j \not\in S} y(j) }\right)$, $\mu_i \geq 0$ for all $i$ and $\mu_i=0$ for $i\notin S$.
		
		\item $\x$ can be computed in $\mathcal{O}(N\log N)$ time.
		
	\end{enumerate}
\end{proposition}



\subsection{The Multiplicative Weight Algorithm}

We propose an algorithm that follows a multiplicative weight strategy (see Algorithm~\ref{alg:SMB1}). We describe here the basic approach given by the mirror descent algorithm. In Section~\ref{sec:Extension} we present an extension of the algorithm that in practice shows a better relation between the allocations and the ratios between the SLAs.
%
\begin{center}
\begin{algorithm}[H]
	\KwIn{Parameters $0<\varepsilon\leq \frac{1}{10}, 0  <\eta < \frac{1}{3} $.}
	%		\KwData{this text}
	%	\KwResult{how to write algorithm with \LaTeX2e }
	Initialization: $\h_1$ any allocation over $\Delta_\varepsilon$ and $\lambda= \frac{\varepsilon^2}{8 N}$. \\
	\For{$t=1,\ldots,T$}
	{
		Set allocation $\h_t$.\\
		Read active and inactive users $A_t$ and $B_t$. $A_t^1=\{ i \in A_t : h_t(i)< \beta(i) \}$, $A_t^2= A_t\setminus A_t^1$. \\
		Set gain function $g_t(i)=\begin{cases}
		1 + \lambda & i \in A_t^1\\
		1  & i\in A_t^2\\
		0  & i \in B_t
		\end{cases}$.\\
		Update allocation:
		\begin{align*}
		\widehat{h}_{t+1}(i) & = h_t(i)e^{\eta g_t(i)}.\\
		\h_{t+1}  &= \pi_{\Delta_\varepsilon}(\widehat{h}_{t+1}).
		\end{align*}
	}
	%\Return $S_k$
	\caption{Multiplicative Weight Update Algorithm} \label{alg:SMB1}
\end{algorithm}
\end{center}
%

Intuitively, the algorithm boosts active users at the expense of inactive ones, and boosts users slightly more if they are currently under their SLA. The algorithm update rule comes from a mirror descent approach applied to a Lagrangian relaxation of a work-maximization linear function at time $t$. More formally, under the assumption that active users have a huge queue, we aim to maximize the objective $\sum_{i\in A_t} w_t(i)$ subject to $w_t(i)\geq \beta(i)$ for $i\in A_t$. The update rule is obtained after applying a mirror descent with a KL-divergence distance generating function over the simplex to the Lagrangian relaxation of the previous problem (see \cite{boyd2004convex,ben2001lectures}). We restrict the projection to the truncated simplex so no user gets an allocation too close to $0$. We use  this update rule solely to guide the algorithm's decisions; however, the proofs of work maximization and SLA satisfaction do not follow from the standard analysis of mirror descent.

%Intuitively, if the decision maker has enough resources to distribute $\left(\sum_{i\in A_t} h_t(i)< 1-\varepsilon\right)$, then she follows a greedy strategy, penalizing users with empty queues. Otherwise, if almost all the resources are being used $\left(\sum_{i\in A_t} h_t(i)\geq 1-\varepsilon\right)$, then she must redistribute the resources in order to satisfy the SLAs, by penalizing the users whose allocation exceeds their SLA. The penalty parameter $ \eta' $ used in the second case is chosen so that these penalties are comparatively less severe than in the first case.


==> version arxiv/Analysis.tex <==
\section{Analysis}\label{sec:Analysis}

To give the analysis of the algorithm and prove Theorem~\ref{thm:main}, we prove the following stronger guarantees about Algorithm~\ref{alg:SMB1}. We compare its performance to the optimal offline dynamic strategy that uses at most a $1-4\varepsilon$ fraction of the resources at each time step.


\begin{theorem}\label{thm:main1}
	Given loads $L_1,\ldots,L_T$, for any $\varepsilon>0$ and $\eta >0$ such that $\varepsilon \leq  1/10$, Algorithm \ref{alg:SMB1} guarantees
	\[
	\work_{\h_1^*,\ldots,\h_{t}^*} - \work_{\text{\textrm{alg}},t} \leq 8\frac{N}{\varepsilon^2 \eta} \ln(N/\varepsilon),
	\]
for any time $1\leq t\leq T$, where $\h_1^*,\ldots,\h_T^*$ is the optimal offline sequence of $(1-4 \varepsilon )$-allocations and $\work_{\text{\textrm{alg}},t}=\sum_{i}\sum_{\tau=1}^t w_{\tau}(i)$ is the work done by Algorithm~\ref{alg:SMB1} until time $t$.
\end{theorem}

The first guarantee of Theorem~\ref{thm:main} regarding work maximization now follows simply from Theorem~\ref{thm:main1}. Given any offline dynamic policy $\h_1,\ldots, \h_T$ such that $\sum_{i}h_t(i)=1$, we define $\bar{\h}_t:= (1-4\varepsilon)\h_t$, which satisfies the assumption of Theorem~\ref{thm:main1}.  Now we have
\begin{eqnarray*}
% \nonumber % Remove numbering (before each equation)
   \work_{\text{alg}} &\geq & \work_{\bar{\h}_1,\ldots,\bar{\h}_T} - 8 \frac{N}{(\varepsilon/4)^2\eta} \ln (4N/\varepsilon) \\
   &\geq & (1-4\varepsilon)\cdot \work_{{\h}_1,\ldots,{\h}_T} - 2000 \frac{N}{\varepsilon^2 \eta} \ln(N/\varepsilon),
\end{eqnarray*}
where the first inequality follows from Theorem~\ref{thm:main1}. To argue the second, let $\w_1,\ldots,\w_T$ and $\overline{\w}_1,\ldots,\overline{\w}_T$ respectively denote the work performed by allocations $\h$ and $\bar{\h}$.
%
%and the second inequality is true by the following argument. The work done by $\h_1,\ldots,\h_T$ is $\work_{\h_1,\ldots,\h_T} = \sum_{i=1}^N\sum_{t=1}^T w_t(i)$ where $\w_1,\ldots,\w_T$ are the work induced by these allocations. On the other hand, the allocations $\overline{\h}_t = (1-4\varepsilon) \h_t$ perform a work $\work_{\overline{\h}_1,\ldots,\overline{\h}_T} = \sum_{i=1}^N \sum_{t=1}^T \overline{w}_t(i)$ where $\overline{\w}_1,\ldots,\overline{\w}_T$ are the work performed by these allocations. How do $\overline{w}_t$ and $\w_t$ compare?. We just need to note that
%
Then $(1-4\varepsilon)\w_1,\ldots,(1-4\varepsilon)\w_T$ are feasible work patterns that the allocations $\overline{\h}_1,\ldots,\overline{\h}_T$ could do, since in this setting we have $1-4\varepsilon$ capacity and the same workload. Therefore, $(1-\varepsilon)\work_{\h_1,\ldots,\h_T} \leq \work_{\overline{\h}_1,\ldots,\overline{\h}_T}$, because the users try to use their allocations at maximum.

%and the second inequality follows since the work done by the dynamic policy $\h_1,\ldots,\h_T$, say $\w_1,\ldots,\w_T$, induces a feasible work $\overline{\w}_1,\ldots,\overline{\w}_T$ under the dynamic policy $\overline{\h}_1,\ldots,\overline{\h}_T$. However, the real work done by policy $\overline{\h}_1,\ldots,\overline{\h}_1$ is at least the work done by $\overline{\w}_1,\ldots,\overline{\w}_T$, which is $(1-\varepsilon)\work_{{\h}_1,\ldots,{\h}_T}$.

Similarly, for SLA satisfaction, we prove a stronger bi-criteria result that implies the SLA guarantee in Theorem~\ref{thm:main}.

\begin{theorem}\label{thm:main2}
	Let $0< \varepsilon\leq 1/10$ and $0< \eta \leq  1/3$. Take any SLAs $\beta(1),\ldots,\beta(N)$ such that $\beta(i) \geq e^{\eta(1+\lambda)} \frac{\varepsilon}{N}$, where $\lambda = \frac{\varepsilon^2}{8N}$ and let $\tilde{p}=32 \frac{N^2}{\varepsilon^3 \eta} \ln (N/\varepsilon)$. Then, for any user $i$ and time $t\leq T-\widetilde{p}$, if we take $\h_1',\ldots,\h_T'$ to be allocations such that $h_t'(i)=\left(1-2\varepsilon\right)\beta(i)$, the work done by Algorithm \ref{alg:SMB1} for user $i$ satisfies
	\[
	\sum_{\tau=1}^{t+\tilde{p}} w_\tau(i) \geq \sum_{\tau = 1 }^t w_\tau'(i),
	\]
	where $\w_t'$ is the work done by the allocations $\h_1',\ldots,\h_T'$. Moreover, $\sum_{\tau=1}^t w_\tau(i) \geq \sum_{\tau=1}^t w_\tau'(i) - \beta(i)\tilde{p}$.
\end{theorem}



\subsection{The Offline Formulation}\label{subsec:LP}


\begin{figure}[t!]
	\centering
	{\small \begin{tabular}{lp{2.5in}|lp{2.5in}}
	$(P_\varepsilon)$ & $  \displaystyle \max \quad\sum_{i=1}^N \sum_{t=1}^T w_t(i) $ & $(D_\varepsilon)$ & $\displaystyle\min\quad  \sum_{i=1}^N \sum_{t=1}^TL_t(i) \gamma_t(i) + (1-\varepsilon)\sum_{t=1}^T \beta_t$ \\
	s.t. & \begin{eqnarray}
	\forall t,i & \sum_{s=1}^t w_s(i)  \leq  \sum_{s=1}^t L_s(i)   \label{eq:const_1} \\
	\forall t & \sum_{i=1}^{N} w_t(i)  \leq  1-\varepsilon   \label{eq:const_2} \\
	\forall t & \quad \w_t  \geq  0
	\end{eqnarray} & s.t. & \begin{eqnarray}
	\forall t,i &  \gamma_t(i) +\beta_t  \geq  1 \\
	\forall t &\gamma_t  \geq  \gamma_{t+1}   \\
	\forall t & \beta_t, \gamma_t  \geq  0
	\end{eqnarray}
	\end{tabular}}
	\caption{The primal and dual LP formulation for the maximum work problem.}\label{fig:LP}
\end{figure}

Before presenting the proof of Theorem~\ref{thm:main1}, we state the offline LP formulation of the maximum work problem for $(1-\varepsilon)$-allocations. We denote by $\w_t=(w_t(1),\ldots, w_t(N) )$ the work done for each user at time $t$. Given loads $L_1,\ldots,L_T$, the offline formulation and its dual LP are given in Figure \ref{fig:LP}. As written, the dual LP includes a change of variable; see Appendix \ref{sec:Omittedproofs} for details.
%\[
%(P_\varepsilon) \begin{array}{rl}
%\max & \sum_{i=1}^N \sum_{t=1}^T w_t(i)\\
%& \begin{array}{rcllr}
%\sum_{s=1}^t w_s(i) & \leq & \sum_{s=1}^t L_s(i) & \forall t,i  & (1) \\
%\sum_{i=1}^{N} w_t(i) & \leq & 1-\varepsilon &\forall t &(2) \\
%\w_t & \geq & 0 & \forall t
%\end{array}
%\end{array}
%\]
Constraints \eqref{eq:const_1} state that the work done for any user up to time $t$ by the allocation cannot exceed the user's loads up to that time. Constraints \eqref{eq:const_2} limit the work performed at time $t$ to at most a $1-\varepsilon$ fraction of the resource.
%\[
%(D_\varepsilon) \begin{array}{rl}
%\min & \sum_{i=1}^N \sum_{t=1}^T \alpha_t(i) \sum_{s=1}^t L_s(i) + (1-\varepsilon)\sum_{t=1}^T \beta_t \\
%& \begin{array}{rcllr}
%\sum_{s=t}^T \alpha_s(i) +\beta_t & \geq & 1 & \forall t,i  & (1') \\
%\alpha,\beta & \geq & 0
%\end{array}
%\end{array}
%\]
%For $(D_\varepsilon)$ we propose the change of variable $\gamma_t(i) = \sum_{s=t}^T \alpha_s(i)$ and, from now on, we will work with the equivalent dual LP %$(D_\varepsilon')$
%\[
%(D_\varepsilon) \begin{array}{rl}
%\min & \sum_{i=1}^N \sum_{t=1}^TL_t(i) \gamma_t(i) + (1-\varepsilon)\sum_{t=1}^T \beta_t \\
%& \begin{array}{rcllr}
%\gamma_t(i) +\beta_t & \geq & 1 & \forall t,i  & (1') \\
%\gamma_t & \geq & \gamma_{t+1} & \forall t \\
%\beta, \gamma & \geq & 0
%\end{array}
%\end{array}
%\]
The LP $(D_\varepsilon)$ will be of special importance in the analysis. Using our algorithm, we will construct a dual feasible solution.

Observe that $(P_\varepsilon)$ is feasible and bounded since the feasible region is a non-empty polytope. Let $v_{P_\varepsilon}$ be the optimal value of $(P_\varepsilon)$. The following proposition gives a simple characterization of $v_{P_{\varepsilon}}$; the proof appears in Appendix~\ref{sec:Omittedproofs}.
%
\begin{proposition}\label{prop:optimalLP}
	$v_{P_\varepsilon} = \min_{0\leq t\leq T} \left(\sum_{s=1}^t \sum_i L_s(i) + (1-\varepsilon)(T-t)\right)$.
\end{proposition}


\subsection{Work Maximization}\label{sec:throughput}

In this section we prove Theorem~\ref{thm:main1}. % Before giving the proof, we will set a series of results about the dynamic generated by algorithm \ref{alg:SMB1}. In what follows, $S_t$ denotes the set of users with tight allocation, that is, $i\in S_t$ if and only if $h_t(i)=\frac{\varepsilon}{N}$. Observe that if user $i\in A_t$ (active), then $h_t(i)=w_t(i)$ since that users has not emptied her queue.
Our first Lemma characterizes the implications of the update rule. The proof follows from a careful analysis of the dynamics using the KL-divergence and appears in Appendix~\ref{sec:Omittedproofs}.

The first result of the lemma shows the behavior of active users' allocations when the system is under-utilized ($\leq 1-\varepsilon$). In this case, all the active users receive a multiplicative boost in their allocation. The second result shows a more general behavior (see also Lemma~\ref{lem:monotonicity2}). In this case, active users with allocation below their SLA do not decrease their allocations while the other active users might decrease their allocation, but in this case, the multiplicative penalization will be less severe.

\begin{lemma}\label{lem:monotonicity}
Let $c=\frac{\varepsilon \eta}{4 N}$. Then Algorithm~\ref{alg:SMB1} satisfies the following:
\begin{enumerate}
\item 	Suppose $\sum_{i \in A_t} h_t(i) \leq  1-\varepsilon$. If $i\in A_t$, then
	$
	h_{t+1}(i) \geq h_{t}(i)(1+c).
	$

\item In general, Algorithm~\ref{alg:SMB1} satisfies $h_{t+1}(i) \geq h_t(i)$ for $i\in A_t^1$ and $h_{t+1}(i)\geq h_t(i) (1-\varepsilon c)$ for $i\in A_t^2$.
\end{enumerate}
\end{lemma}

%\begin{remark}
%	Observe that the assumption $\sum_{i\in A_t} h_t(i)<1-\varepsilon$ is crucial to obtain a multiplicative rate, specially, in the case $B_t\subseteq{S_{t+1}}$.
%\end{remark}

%\begin{proposition}
%	{\color{red} Not used anymore} Suppose $\sum_i \w_t(i) < 1-\varepsilon$. For $t\geq 1$, if $i\in  S_{t+1}$, then $h_t(i)\leq \frac{\varepsilon}{N}e^\eta$.
%\end{proposition}

%\begin{proof}
%	Indeed, by previous parts we know that $e^{\lambda-1} \geq 1$ and therefore, for $i\in S_{t+1}$, we have
%	\begin{align*}
%	\frac{\varepsilon}{N} &= \widehat{h}_{t+1}(i) e^{\mu_i +\lambda-1} \\
%	& \geq \widehat{h}_{t+1}(i) \\
%	& = h_t(i) e^{-\eta}
%	\end{align*}
%	which implies the result.
%\end{proof}


%\begin{lemma}\label{lem:badtime2}
%	{\color{red} Not used anymore} Suppose $\sum_i \w_t(i) < 1-\varepsilon$. Suppose that $B_t\subseteq S_{t+1}$, then $\sum_{i} \w_t(i) \geq 1- e^{\eta}\varepsilon$.
%\end{lemma}

%\begin{proof}
%	Recall that $h_t(i) = \w_t(i)$ for $i\in A_t$, then
%	\begin{align*}
%	\sum_i \w_t(i) & \geq \sum_{i\in A_t} h_t(i) \\
%	& = 1 - \sum_{i\in B_t} h_t(i) \\
%	& \geq 1 - e^{\eta} \frac{\varepsilon}{N} |B_t|\\
%	& \geq 1-\varepsilon e^\eta.
%	\end{align*}
%\end{proof}

%This last lemma says that if the algorithm is doing little work, but all penalized users go into the threshold allocation, then, the algorithm work was just below $1-\varepsilon$.

%Now, let $D_t = \{ i : h_t(i) \leq \beta(i)  \}$ and $U_t = [N]\setminus D_t$ be the set of users under their SLA and the set of users over their SLA, respectively. The following results states that if the algorithm is doing enough work, then, the penalized users do not decrease their allocation abruptly.

%\begin{lemma}\label{lem:monotonicity2}
%	For $\varepsilon< 1/10$ and $\eta\geq 0$, take $\eta'\geq 0$ such that $e^{\eta'}= 1+ \frac{\varepsilon^2}{N}(1-e^{-\eta}) \geq 1$. Suppose $\sum_{i\in A_t} h_t(i)\geq 1-\varepsilon$. If $i \in U_t$, then
%	\[
%	h_{t+1}(i) \geq h_t(i) (1- 2\varepsilon c),
%	\]
%	where $c=\frac{\varepsilon}{N}(1-e^{-\eta})$ is defined in lemma \ref{lem:monotonicity}.
%\end{lemma}


%We now focus on proving that algorithm \ref{alg:SMB1} performs well in throughput.



\begin{proof}[Proof of Theorem~\ref{thm:main1}]
Given loads $L_1,\ldots,L_T\in \R_+^N$, consider the following $\{0,1\}$-matrix $M$ of dimension $N\times T$ that encodes the information about the status of queues obtained while running Algorithm~\ref{alg:SMB1}
\[
M_{i,t} = \begin{cases}
0 &i\text{'s queue is empty at }t, Q_t(i)=0,\\
1 & i\text{'s queue is not empty at }t, Q_t(i)>0.
\end{cases}
\]

Let $\widetilde{s}=\frac{\ln (N/\varepsilon)}{\varepsilon c}$, where $c$ is defined in Lemma~\ref{lem:monotonicity}. Now, pick $s^\star$ to be the maximum non-negative integer $s$ (including $0$) such that
\begin{equation}\label{eq:switch2}
\sum_{t=1}^{s} \sum_{i} L_t(i) \leq \sum_{t=1}^{s+\widetilde{s}} \sum_{i} w_t(i)
\end{equation}

\begin{claim}\label{cl:gooduser1}
	Consider any block of time $[r,r+\tilde{s}]$ where $r> s^{\star}$; then there exists a user $i$ such that $M_{i,r'}=1$ for all $r'\in [r,r+\tilde{s}]$.
\end{claim}
\begin{proof}
	Suppose not. Then we claim that $s=r$ satisfies condition \eqref{eq:switch2}. Consider any user $i$ and let $r'_i\in [r,r+\tilde{s}]$ be such that $M_{i,r'_i}=0$. Then work done by the user $i$ up to time $r+\tilde{s}$ is at least
	$$\sum_{t=1}^{r+\tilde{s}}  w_t(i)\geq \sum_{t=1}^{r'_i}  w_t(i)= \sum_{t=1}^{r_i'}  L_t(i)\geq \sum_{t=1}^{r}  L_t(i).$$
	Now summing over all $i$, we get the desired contradiction.
\end{proof}



We now prove the following claim that shows that the algorithm ensures that, on average, the total resource utilization after $s^\star$ is close to $1-4\varepsilon$. The proof of the Claim relies on Lemma~\ref{lem:monotonicity} and appears in Appendix~\ref{sec:Omittedproofs}.
\begin{claim}\label{cl:gooduser2}
	Let $B=[r,r+\tilde{s})$ with $r>s^\star$ be a consecutive block of $\tilde{s}$ timesteps and let $B'=\{  t \in B :  \sum_{j\in A_t} h_t(j) \leq 1- \varepsilon  \}$ be the time steps in $B$ with low utilization. Then $|B'|\leq 4\varepsilon \tilde{s}$ and therefore,  $\sum_{t=s^\star +1}^T \sum_i w_t(i)  \geq ( 1 - 4 \varepsilon )(T-s^\star) -\widetilde{s}.$
\end{claim}


Now, consider the following feasible dual solution of $(D_{4\varepsilon})$: $\gamma_t(i)=1,\beta_t=0$ for all users $i$ and $t=1,\ldots,s^\star$, and $\gamma_t(i)=0, \beta_t=1$ for all users $i$ and $t=s^\star+1,\ldots,T$. Observe that $\sum_{t=1}^T \beta_t = T-s^\star$. For optimal $(1-4 \varepsilon)$-allocations $\h_1^*\ldots,\h_T^*$ we obtain
	\begin{align*}
	\work_{\h_1^*,\ldots,\h_T^*} & \leq v_\text{dual}(\gamma_1,\ldots,\gamma_T,\beta_1,\ldots\beta_T) \tag{weak duality} \\
	&= \sum_{t=1}^{s^\star}\sum_i L_t(i) + (1-4 \varepsilon)(T-s^\star)\\
	& \leq \sum_{t=1}^{s^\star + \widetilde{s}} \sum_i w_t(i) + (1-4 \varepsilon)(T-s^\star) \tag{choice of $s^\star$}\\
	& \leq \sum_{t=1}^{s^{\star}}  \sum_i w_t(i) + \widetilde{s} + \sum_{t=s^{\star}+1}^{T}\sum_i w_t(i) + \widetilde{s} \tag{Claim \ref{cl:gooduser2}}\\
	%& = \sum_{t=1}^T \sum_i w_t(i) + \sum_{t=s^\star+1}^{s^{\star}+s'}\sum_i w_t(i) + \widetilde{s}\\
	%& \leq \work_{\text{alg}} + (N+1)\widetilde{s} \tag{$\sum_iw_t(i)\leq 1$}\\
	%& = \work_{\text{alg}} + (N+1) \frac{\ln (N/\varepsilon)}{\varepsilon c} \tag{$\widetilde{s}= \frac{\ln(N/\varepsilon)}{\varepsilon c}$} \\
	& = \work_{\text{alg}} + 8\frac{N}{\varepsilon^2 \eta} \ln(N/\varepsilon).
	\end{align*}
where we have used $\sum_{t=s^\star+1}^{s^\star+\widetilde{s}} w_t(i) \leq \widetilde{s}$ and the definition of $\widetilde{s}$. %$\tag{$c= \frac{\varepsilon}{N}(1-e^{-\eta})$}$
\end{proof}












%%%%%% SLA Satisfaction


\subsection{SLA Satisfaction}\label{sec:SLAsat}

In this section, we prove Theorem~\ref{thm:main2}. Recall that $\lambda = \frac{\varepsilon^2}{8N}$ and $A_t^1=\{ i\in A_t: h_t(i)<\beta(i)  \}$ is the set of active users receiving less than their SLAs and $A_t^2=A_t\setminus A_t^1$ is the set of active user receiving at least their SLA. Analogous to Lemma~\ref{lem:monotonicity}, we have the following lemma, whose proof appears in Appendix~\ref{sec:Omittedproofs}.

\begin{lemma}\label{lem:monotonicity2}
	Assume $\varepsilon \leq \frac{1}{10}$, $\eta\leq \frac{1}{3}$ and $\beta(i)\geq 2\frac{\varepsilon}{N}$ for all users. Then for any $i\in A_t^1$, Algorithm~\ref{alg:SMB1} guarantees $h_{t+1}(i)\geq h_t(i)(1+c')$, where $c'= \frac{\varepsilon\eta \lambda}{2N}$.
\end{lemma}




\begin{proof}[Proof of Theorem \ref{thm:main2}]
	Let $\widetilde{p}= \left\lceil\frac{\ln(N/\varepsilon)}{\ln(1+c')} \right\rceil$, where $c'$ is defined in Lemma~\ref{lem:monotonicity2}. Now, we proceed by induction on $t$ to prove that $\sum_{\tau=1}^{t+\widetilde{p}} w_\tau(i) \geq \sum_{\tau=1}^t w_\tau'(i)$, where $\w_t'$ is the work done by the allocations $\h_1',\ldots,\h_T'$. Clearly, the case $t=0$ is direct.
	
	Take $t\geq 1$ and suppose the result is true for $t-1$. If there exists $r\in[t, t+\widetilde{p}]$ such that user $i$'s queue is empty, then
	\[
	\sum_{\tau=1}^{t+\widetilde{p}} w_\tau(i) \geq \sum_{\tau=1}^{r} w_{\tau}(i) = \sum_{\tau=1}^{r}  L_\tau(i) \geq \sum_{\tau=1}^t w_\tau'(i).
	\]
	Therefore, assume that for all $\tau \in [t,t+\widetilde{p}]$ we have that user $i$'s queue is non-empty. By the induction hypothesis
	\[
	\sum_{\tau=1}^{t-1+\widetilde{p}} w_t(i) \geq  \sum_{\tau=1}^{t-1} w_\tau'(i).
	\]
	In order to complete the proof, we need to prove that  $w_{t+\widetilde{p}}(i) \geq w_t'(i)$. We proceed as follows. Suppose that for all $\tau\geq t$ we have $ w_\tau(i)< (1-\varepsilon)\beta(i)$. By Lemma~\ref{lem:monotonicity2}, at each time $\tau \in [t,t+\widetilde{p}]$ the allocation of user $i$ increases multiplicatively by a rate $(1+c')$. Therefore,
	\[
	w_{t+\widetilde{p}}(i) \geq \frac{\varepsilon}{N}(1+c')^{\widetilde{p}} \geq 1 \geq \beta(i),
	\]
	a contradiction. From the previous analysis we obtain the existence of $\tau^\star\in [t,t+\widetilde{p}]$ such that $w_{\tau^\star}(i)\geq (1-\varepsilon) \beta(i)$. By using Lemmas \ref{lem:monotonicity} and \ref{lem:monotonicity2}, we can show that the allocation $h_\tau(i)$ will never go below $(1-\varepsilon c)(1-\varepsilon)\beta(i)$ for all $\tau\geq \tau^\star$. In particular $w_{t+\widetilde{p}}(i)\geq (1-\varepsilon c)(1-\varepsilon)\beta(i) \geq (1-2\varepsilon)\beta(i) \geq w_t'(i)$.
\end{proof}

%
%\begin{corollary}
%	Fix $\eta \geq 1$. For any user $i$ take any $\h_1',\ldots,\h_T'$ $1$-allocations such that $h_t(i)= \beta(i)$. Then, for all time $t$ we have
%	\[
%	\sum_{\tau=1}^{t} w_\tau'(i) - \sum_{\tau=1}^t w_\tau(i) \leq \mathcal{O}(N^{6/5} t^{3/5} \ln (N t)).
%	\]
%\end{corollary}
%
%\begin{proof}
%	Observe that $\h_t'' = (1-\varepsilon c) \h_t'$ is a $(1-\varepsilon c)$ allocation such that $h_t(i)''= (1-\varepsilon c)h_t(i)'$. Therefore, we can apply theorem \ref{thm:main2} and obtain
%	\[
%	\sum_{\tau = 1}^{t+s} w_\tau(i) \geq \sum_{\tau =1 }^t w_\tau''(i)
%	\]
%	where $\w_\tau''$ is the work done by the allocation $\h_1'',\ldots, \h_T''$. Moreover, It is easy to see that $w_t''(i) \geq (1-\varepsilon c)w_\tau'(i)$. Then
%	\[
%	\sum_{\tau = 1}^t w_t'(i)-\sum_{\tau = 1}^{t} w_\tau(i) \leq   \varepsilon c t + s.
%	\]
%	Since $s\leq 2 \frac{\ln (N/\varepsilon)}{\ln (1+c')}\leq 8 \frac{N^2}{\varepsilon^3}\ln(N/\varepsilon)$ we conclude by taking $\varepsilon = \frac{N^{3/5}}{t^{1/5}}$.
%\end{proof}



==> version arxiv/Conclusions.tex <==
\section{Conclusion}
\label{sec:Conclusions}

We have proposed a new online model for dynamic resource allocation of a single divisible resource in a shared system. Our framework captures basic properties of cloud systems, including SLAs, limited system feedback and unpredictable (even adversarial) input sequences. We designed an algorithm that is near-optimal in terms of both work maximization and SLA satisfaction (Theorems~\ref{thm:main}, \ref{thm:mainextension} and \ref{thm:SLAextension}). Furthermore, our second algorithm, Algorithm~\ref{alg:SMB2}, can be applied in an over-commitment regime with similar guarantees, which could be of additional merit for some applications. We derived a simple expression for the offline work maximization problem that allowed us to reinterpret the algorithm's dynamics as an approximate solution of the optimal (offline) work maximization LP. Numerical experiments show that our algorithm is indeed able to achieve a desirable trade-off between work maximization and SLA satisfaction. In particular, comparisons with offline algorithms (PG and restPG) indicate that our algorithm is empirically work maximizing. Further, unlike other plausible online algorithms, our algorithm is able to quickly adapt to unexpected changes in demand and still approximately satisfy the underlying user SLAs.
%
Our model and results may be extended in various directions of interest to the operations research and cloud computing communities. %Some potential future directions include exploiting predictions about future workloads (as in \cite{lykouris2018competitive}), and simultaneously allocating multiple resources. %ATH: I feel like this could be fleshed out, but only if we cut down elsewhere.

A natural extension for single-resource systems is to model priority among users. Typically, users with higher priority should be given resources before their lower-priority counterparts. A challenge in this setting is how to define the metric corresponding to work maximization. One possibility is to have different weights for different users, corresponding to their priority, and then to maximize the weighted total work while satisfying SLAs. %The challenge of obtaining an algorithm that optimizes both a weighted total work done as well as individual SLAs remains open.
Directly extending our algorithms to this case means a user's multiplicative boost depends on their priority. However, our analysis in this paper does not apply, as we use the fact that users' work is interchangeable, whereas the identity of who performs the work is critical in the prioritized case.
%This can be modeled by adding weights to each user's work with the aim to maximize the weighted work done while hold SLA satisfaction. Applying the same Lagrangian relaxation to this problem as we did in Section~\ref{sec:Analysis} we obtain a multiplicative weight algorithm with multiplicative boost depending on the users' weights. However, this new method has proven unstable in the following way. Large multipliers for correcting users with allocations below SLA give poor work comparison. On the other hand, small multipliers for this case yield poor SLA satisfaction. The unweighted case does not exhibit this ill-behavior since the work performed by any users is in some sense exchangeable while in the weighted case it is critical who performs the work at each time.


Another challenging extension is the management of multiple resources (e.g., CPU, I/O bandwidth, memory), where different users or jobs may require the resources in different proportions. This extension requires a fundamental redefinition of our model, where work done for a user is a function of the multiple resources allocated, and may also depend on a particular job's characteristics. In many real-world scenarios, a job's resource demands are often complementary, e.g.\ RAM and CPU usage. This observation may motivate a possible extension in which we still treat all users' loads as one-dimensional quantities, and the work performed by a user is a relatively simple function of their allocations, e.g.,  a concave non-decreasing function.

%
%We need to link the usage of resources according to the (unknown) users' demand. For simplicity, we assume the work performed is proportional to the job's demand pattern and the available resources. To understand this, assume there are two (divisible) resources. Intuitively, if the demand of user $i$ at time $t$ is the resource-pair $L_t(i)= (0.1,0.3)$, the work performed by user $i$ is going to be proportional to $0.1:0.3= 1:3$ of the user's allocated resources, that is, every unit of resource $1$ and $3$ units of resource $2$ allow us to perform $1$ unit of work (in this pattern). Incomplete demand goes to the queue as usual. In this more realistic scenario, we need to model demand via batches, where batches model the different job's resource requirements. The next batch is processes after the previous batch has been completed. Since the work done is a multidimensional vector, we need to redefine our objective. A naive one is to minimize the batch delay while simultaneously ensure SLA satisfaction for each user and resource. We can still apply our algorithm (one for each resource). However, suffering from batch delay due to resource bottleneck seems unavoidable. More discouraging is the fact that assigning resources without observing the batch pattern might result in a situation where all the users block themselves cyclically, e.g., consider a system with two users with pair of SLAs $\beta(1)=(0.1,0.9)$ and $\beta(2)=(0.9,0.1)$ and constant pattern $L_t(i)=(0.5,0.5)$ for both of them. After a while, our approach will assign to each user their SLAs with a performance of roughly $(0.1,0.1)$ at each time, yet $(0.5,0.5)$ is a better allocation $(0.5,0.5)$ for each of them which ensures SLA satisfaction and no batch delay.}

%One possible future direction is to extend the objective to capture additional natural properties of shared systems. Right now, we ensure high utilization and SLA satisfaction. However, in practice, each user can have a priority in the system where high-priority users may obtain resources faster than low-priority users. One way to model this is by weighting users and the new objective is to maximize the weighted work done by the algorithm and keep satisfying SLAs. Nonetheless, we cannot hope for a fair comparison against the best offline allocations (as we did in this work) because the best offline solution for the weighted case is the one that allocates greedily by starting from the user with highest priority. This issue was not present in this work (unweighted case) since the work done by each user was in some sense exchangeable. One way to bypass this is by restricting the benchmark to offline allocations that guarantee a constant fraction of the SLA for each user.
%
%Another direction is to extend the model to multiple resources. In real applications, different jobs complement the use of multiple resources such as CPU, memory or I/O bandwidth. For this reason, the task of extending the model to multiple resources presents further challenges. One way to do it is by setting a model of resources that behave in a CPU-style, that is, users' work is proportional to their allocations. In this model, users' loads are divided into batches, where each user's batch represents a process with a constant but unknown resource requirements, called the \emph{pattern} of the batch. A new batch is loaded only when the previous one was completely processed by the system. Users perform work proportional to their current batch pattern trying to do as much work as their allocations allows them to do. For each resource we also have an SLA per user. Clearly, we can suffer from batch delay processing time due to resource bottleneck. In this model, one goal is to design small-delay algorithms and at the same time guarantee SLA satisfaction.
%
%Finally, in our model, we have assumed that SLA satisfaction is enough to guarantee user contentment. However, we do not know if SLA satisfaction corresponds to the right objective from a \emph{fairness} or \emph{game-theoretic} point of view. 

==> version arxiv/Experiments.tex <==
\section{Experiments}\label{sec:Numerical}

In this section, we empirically test Algorithm~\ref{alg:SMB2} against a family of offline and online algorithms. We aim to measure the performance on both synthetic data as well as real CPU traces from a production service in Microsoft's cloud. We quantify the performance on the following three criteria.


% In the first subsection, we aim to measure the theoretical guarantees given in Theorem~\ref{thm:main} by constructing a random sequence of loads of the order of million time steps. For work-maximization, we compare the cumulative work done by Algorithm~\ref{alg:SMB2} against the cumulative work done by optimal offline solution and the optimal offline solution restricted to $(1-\varepsilon)$ resource. Likewise, we test SLA satisfaction by comparing individual queue lengths as in Corollary~\ref{cor:Queues}. Even though we do not explicitly give any guarantee with respect to the $2$-norm of queues, we empirically show remarkably results with this metric. Also, this metric will be of importance in the next set of experiments aimed to compared Algorithm~\ref{alg:SMB2} against other reasonable and simple online algorithms.

%In the next subsection, we use real CPU traces of a production service in Microsoft's cloud to test Algorithm~\ref{alg:SMB2}. Once more, we run tests for work maximization, SLA satisfaction and queue length. However, since the data is shorter than in the previous experiment, we use an \emph{instantaneous SLA satisfaction} metric which is aimed to test the performance of Algorithm~\ref{alg:SMB2} against the static SLA policy but in a short time window of time.
\begin{itemize}
	\item \textbf{Work maximization.} We compare the overall work done by Algorithm~\ref{alg:SMB2} against various benchmark algorithms.
%	\item Individually, we compare the cumulative work done by each user in Algorithm~\ref{alg:SMB2} with the work done by \emph{Proportional Greedy} (Algorithm~\ref{alg:PropGreedy} below).
	
	\item \textbf{SLA guarantee.} We examine the extent to which our algorithm achieves the cumulative work of the static SLA policy for each user. We do so by measuring the cumulative work over plausible time windows.

%should be close to the work done under the static SLA policy. {\color{red}This means that there shouldn't exist long periods of time where an active user do little work. We present empirical tests that show that Algorithm~\ref{alg:SMB2} is able to ensure a quality of service comparable to the static SLA policy in few steps.}
	%	We compare the individual queues for each user given by Algorithm~\ref{alg:SMB2} versus the queues given by the benchmark algorithms. There is a one-to-one relation between work done and queue length as Corollary~\ref{cor:Queues} suggests. This result states that the latency of each user should be comparable to the latency of the static SLA policy for long enough time windows. For this reason, we study the individual queue lengths instead of the cumulative work. For the purpose of SLA satisfaction, we only need to compare against the static SLA allocation. However, we also show the behavior of other benchmark algorithms.
	
	\item \textbf{Queue length.} We compare the $2$-norm of the individual queues over time. %given by Algorithm~\ref{alg:SMB2} against the queues given by the benchmark algorithms.
 We use this metric as a proxy for the system latency, which is not captured by our theoretical results. % However, experiments suggest positive results for Algorithm~\ref{alg:SMB2}.
\end{itemize}



%{\color{red}There was a discussion about queues in SLA. Put that is queues, if at all.}


We consider the following \emph{online algorithms}, against which we benchmark our algorithm.
%
\begin{itemize}
\item \textbf{Static SLA Policy (Static)}. Each user gets their SLA as a constant, static allocation. We call this algorithm Static.

\item \textbf{Proportional Online (PO)}. In each iteration, every active user will get their SLA normalized by the sum of SLAs of active users (just their SLA if there are no active users). This simple algorithm seems suitable for a practical implementation; however, its performance can be arbitrarily bad in terms of work maximization. The formal description appears in Algorithm~\ref{alg:OnlProp} in Appendix~\ref{sec:Add_Alg}. We call this Algorithm PO.

\item \textbf{Online Work Maximizing (OWM)}. This algorithm divides users into three categories: $A,B$ and $I$ (active users with allocation, actives users without allocation and inactive users). At each iteration, the resource is divided uniformly among users in $A$. If a user in $A$ becomes inactive, they are moved to $I$. If a user in $I$ becomes active, they are moved to $B$. When $A$ becomes empty, we move all users from $B$ to $A$. In Appendix~\ref{sec:localgreedy} we prove that this method is work maximizing. However, this greedy strategy is not guaranteed to satisfy SLA constraints for general input loads. We call this algorithm OWM.
\end{itemize}
%
%
We also consider the following \emph{offline algorithms}, against which we benchmark our algorithm. %Observe that offline algorithms are very stringent measures, nonetheless, we compare the performance of our algorithm against offline algorithms as also has been done in the theoretical results.
%
\begin{itemize}
\item[*] \textbf{Optimal $1$-allocations (PG)}. The optimal offline solution to the work maximization problem. This solution is computed using Algorithm~\ref{alg:PropGreedy}, which we call Proportional Greedy (PG). This algorithm can be considered as the offline counterpart of Proportional Online.

\item[*] \textbf{Optimal $(1-\varepsilon)$-allocation (restPG)}. Offline solution to the work maximization problem with resource restricted to $1-\varepsilon$, where $\varepsilon$ is the parameter of Algorithm~\ref{alg:SMB2}. %We compute this solution with a restricted version of Proportional Greedy.
\end{itemize}


\subsection{Synthetic Experiment}
%
%Our experimental goal is testing the effectiveness of the extension described by Algorithm~\ref{alg:SMB2} and comparing the theoretical guarantees developed for our model. Theorem~\ref{thm:mainextension} establishes that the work done by Algorithm~\ref{alg:SMB2} is at least the optimal work done by $(1-\varepsilon)$-allocations plus a constant additive error independent of the time horizon. In terms of SLA guarantee, Theorem~\ref{thm:GeneralLB_main} states that Algorithm~\ref{alg:SMB2} produces individual work comparable to $(1-\varepsilon)$ times individual SLAs.
%
%
%In this section, we display various comparison that show Algorithm~\ref{alg:SMB2}'s robustness in practice. We will consider the following measurements:
%\begin{itemize}
%	\item \textbf{Work maximization.} We compare the overall work done by Algorithm~\ref{alg:SMB2} and the overall optimal work done by $1$-allocations. We also compare the overall optimal work done by $(1-\varepsilon)$-allocations. In this experiment we expect to outperform the work done by $(1-\varepsilon)$-allocations and to be slightly surpassed by the work done by the optimal $1$-allocations. Numerical experiments corroborate this statement.
%	
%%	\item Individually, we compare the cumulative work done by each user in Algorithm~\ref{alg:SMB2} with the work done by \emph{Proportional Greedy} (Algorithm~\ref{alg:PropGreedy} below).
%	
%	\item \textbf{SLA guarantee.} We compare the queues of Algorithm~\ref{alg:SMB2}, the queues of Proportional Greedy and Proportional Static Allocations (see below for details). The latter is a more demanding criterion than the usual comparison against static SLAs. Later, we empirically observe that Algorithm~\ref{alg:SMB2} performs extremely well against these two methods. We show that in the long term active users converge to their proportional allocation given by their SLAs. For completeness we show the behavior of Proportional Greedy but with allocations moderately constrained.
%	
%	\item \textbf{Queue length.} Finally, we compare the $2$-norm of the queues of Algorithm~\ref{alg:SMB2}, Proportional Greedy and Proportional Static Allocations. With this we aim to measure the variance of the overall queues. Again, for completeness we empirically show the $2$-norm of the queues of a slightly constrained Proportional Proportional Greedy solution. We remark that we do not have any theoretical guarantee with respect to this metric. However, experiments suggest positive results for Algorithm~\ref{alg:SMB2}.
%\end{itemize}
%
%In what follows, to compute the optimal offline allocation we use an offline algorithm that we call \emph{Proportional Greedy}, depicted in Algorithm~\ref{alg:PropGreedy}. It is easy to see that the algorithm is work maximizing. Moreover, for any time $t$, all \emph{active} users' allocations are pairwise proportional to their SLAs and at least their SLA. Indeed, in Algorithm~\ref{alg:PropGreedy}, every time we remove an active user (line 9), the potential proportional share of the remaining users can only increase. Since the minimum share is the SLA, the property follows.
%
%%Indeed, observe that at each time there are two kind of updates: the first one (line 9 in Algorithm) eliminates a user of the current active set $A$; the second one (line 13 in Algorithm) distributes the remaining resources $\mathrm{Rem}$ among the active users whenever the remaining work for each user $i\in A$ is at least $\frac{\beta(i)}{\sum_{j\in A}} \mathrm{Rem}$. Observe that when an update of type one occurs we eliminate an user $i^*$ and the potential proportional share that the rest of the active users $A\setminus\{ i^* \}$ increases. This ensures that each time an update of type one occurs, the allocation given to active users cannot decrease. The minimum possible share is always the SLA. At the end, active users get at least their SLA and between them, pairwise their share proportional SLAs.
%
%For the (piecewise) static allocation policy, we consider the (piecewise) \emph{Proportional Static Allocation} (PSA) defined as follows. The time is partitioned into periods. In each period a subset of users will assume the role of \emph{active users} (even if they actually do not demand any resource). Let us call that set of users $S$. The static allocation during that period will be proportional to $\frac{\beta(i)}{\sum_{k\in S}\beta(k)}$ for users in $S$ and $0$ otherwise. The choice of this allocations will be clear after we explain how the demands are set. Observe that if $|S|=N$, then we obtain $\beta(i)$ for all users.
%
%%For simplicity, from now on, we refer to Algorithm~\ref{alg:SMB2} as the \emph{Online Algorithm}.
%
%\begin{center}
%	\begin{algorithm}[H]
%		\KwIn{Sequence of loads $(L_t)_{t=1}^T$ and SLAs $\beta(1),\ldots,\beta(N)$.}
%		%		\KwData{this text}
%		%	\KwResult{how to write algorithm with \LaTeX2e }
%		%Set allocation $\h_1$.\\
%		\For{$t=1,\ldots,T$}
%		{
%			$w_t(i) \leftarrow 0$, $\forall i\in [N]$. \\
%			$\mathrm{Rem} \leftarrow 1$.\\
%			$\mathrm{Rem}(i) \leftarrow Q_{t-1}(i) + L_t(i)$, $\forall i \in [N]$. \\
%			\Repeat{$\mathrm{Rem}=0$ or $\{ i : \mathrm{Rem}(i)> 0 \}= \emptyset$}{
%				$A \leftarrow \{  i : \mathrm{Rem}(i) >0  \}$.\\
%				$\Sigma \leftarrow  \sum_{i\in A_t} \beta(i)$.\\
%				$i^*\leftarrow \argmin_{k\in A} \mathrm{Rem}(k) $.\\
%				\If{$\mathrm{Rem}(i)< \frac{\beta(i)}{\Sigma} \mathrm{Rem} $}{
%					$w_t(i^*)\leftarrow w_t(i^*)+ \mathrm{Rem}(i^*)$.\\
%					$\mathrm{Rem} \leftarrow \mathrm{Rem} - \mathrm{Rem}(i^*)$.\\
%					$\mathrm{Rem}(i^*)\leftarrow 0$.
%				}
%				\Else{
%					\For{$k\in A$}{
%						$w_t(k) \leftarrow w_t(k) + \frac{\beta(k)}{\Sigma}  \mathrm{Rem}$.\\
%						$\mathrm{Rem}(k) \leftarrow \mathrm{Rem}(k) - \frac{\beta(k)}{\Sigma}  \mathrm{Rem}$.
%					}
%					$\mathrm{Rem} \leftarrow 0.$
%				}
%			}
%		}
%		%\Return $S_k$
%		\caption{Proportional Greedy} \label{alg:PropGreedy}
%	\end{algorithm}
%\end{center}


\subsubsection{Description of the Experiment}~
In this experiment, we consider a synthetically generated input sequence, which we use to examine how online algorithms adapt to different conditions. %Intuitively, the demands are constructed in a way that they can affect at different times either the total-work objective or the SLA satisfaction requirement}. %ATH: Not sure this sentence adds much.
Specifically, our system consists of three users with SLAs of $\beta(1) = 0.2$, $\beta(2)=0.3$ and $\beta(3) = 0.5$. We consider a time horizon of $T=3,\!000,\!000$. The load input sequence is divided into six periods: $P_i=\left[ \frac{(i-1)T}{6},  \frac{iT}{6} \right)$ for $i=1,\ldots,6$. In each period, only two users demand new resources. During the first $3$ periods, the random demand has a mean proportional to the users' SLA. In the following $3$ periods, the random demand changes to a distribution with uniform mean among users demanding resources. Specifically:
\begin{itemize}
	
\item During $P_1$, only users $2$ and $3$ demand the following loads. At the beginning of $P_1$, %\im{What do you mean by at the first time?}
i.e., $t=1$, user $2$ demands a large load of $L_1(2) \sim \frac{T}{6}\cdot \mathrm{Gamma}\left(2000, \frac{1}{2000}\cdot\frac{\beta(2)}{\beta(2)+ \beta(3)} \right)$ and $L_1(3)=0$. During the rest of period $P_1$, $L_t(2)=0$ and $L_t(3) %= \frac{T/6}{T/6-1}\cdot % ATH: Made this correction; seems like having this factor here is a typo, right?
\sim \mathrm{Gamma}\left(2000, \frac{1}{2000}\cdot\frac{\beta(3)}{\beta(2)+ \beta(3)} \right)$. User $1$ demands nothing during this entire period. Similar loads are set for period $P_2$ and $P_3$. %During $P_2$, users $1$ and $2$ demand  loads $L_t(i)=X_t(i)\sim \mathrm{Gamma}\left(2000, \frac{1}{2000}\cdot\frac{\beta(i)}{\beta(1)+ \beta(2)} \right)$ and $L_t(3)=0$. Finally, during $P_3$, users $1$ and $3$ demand loads $L_t(i)=X_t(i)\sim \mathrm{Gamma}\left(2000, \frac{1}{2000}\cdot\frac{\beta(i)}{\beta(1)+ \beta(3)} \right)$ and $L_t(2)=0$.
	
\item Similarly, during $P_4$ users $2$ and $3$ demand $L_t(i) \sim \mathrm{Gamma}\left(2000, \frac{1}{2000}\cdot \frac{1}{2}\right)$ for $i=2,3$. During $P_5$ users $1$ and $2$ demand $L_t(i) \sim \mathrm{Gamma}\left(2000, \frac{1}{2000}\cdot \frac{1}{2}\right)$ for $i=1,2$. During $P_6$ users $1$ and $3$ demand $L_t(i) \sim \mathrm{Gamma}\left(2000, \frac{1}{2000}\cdot \frac{1}{2}\right)$ for $i=1,3$.
	
\end{itemize}


%Recall that a Gamma distribution is characterized by two parameters: the \emph{shape} $k> 0$ and the \emph{scale} $\theta> 0$. The PDF of a Gamma$(k,\theta)$ is given by $\frac{1}{\Gamma(k) \theta^k} x^{k-1} e^{-x/\theta} $ where $\Gamma(k)= \int_{0}^{\infty} u^{k-1} e^{-u} \mathrm{d}u$ is the standard Gamma function. See Figure~\ref{fig:gammaplot} for PDFs of different Gamma distribution for various choices of $k$ and $\theta$.
%
%\begin{figure}[h!]
%	\centering
%	\includegraphics[width=0.75\linewidth]{figures/Gamma_plot-1}
%	\caption{PDF of different Gamma distributions.}
%	\label{fig:gammaplot}
%\end{figure}

The expectation of a Gamma$(k,\theta)$ random variable is given by $k\theta$ and the variance is given by $k\theta^2$ (see e.g.\ \cite{feller1957introduction}). For example, in period $P_1$ user $2$'s expected load is $ \frac{T}{6} \frac{\beta(2)}{\beta(2)+\beta(3)}$, with variance $\frac{1}{2000} \left( \frac{\beta(2)}{\beta(2)+\beta(3)} \right)^2$. Similarly, user $3$'s expected total load is $ \frac{T}{6} \frac{\beta(3)}{\beta(2)+\beta(3)}$. Thus, the expected overall load is $T/6$, exactly the length of the period. %{\color{red}These loads are set in order to benefit online algorithms that are work maximizing or ensure proportional SLA allocations (OWM, PO). However, the first large load will hurt OWM in SLA satisfaction (see below). This is also the case for periods $P_2$ and $P_3$. In the last three periods, $P_4,P_5$ and $P_6$, we drastically change the distributions to hurt algorithm PO. Again, the overall work during each period will be $T/6$ but it will not be a multiple of SLA.} \im{not clear}.
 A brief summary of Gamma distribution's properties is given in Appendix \ref{sec:Gamma}.

%{\text{red} check this again}

%We slightly constraint the Gamma random load by $(1-\varepsilon/3)$. The reason for this is because in each period only two users demand new resources and Algorithm~\ref{alg:SMB2} always reserves a small amouunt of $\varepsilon'/N$ resource for each user, where $\varepsilon'$ is the parameter of the algorithm. So in order to make the comparison \emph{fairer} against Algorithm~\ref{alg:SMB2} solution we restrict the loads to $(1-\varepsilon/3)$ in expectation.

%{\text{remove Proportional Static Allocation}}

%Now, Proportional Static Allocation is set according to users demanding resources in each period. For instance, in period $P_2$ only user $1$ and $2$ demand  new resources, so Proportional Static Allocation allocates $(1-\varepsilon/3) \frac{\beta(i)}{\beta(1)+\beta(2)}$ for $i=1,2$ and $0$ for user $3$.

We instantiate Algorithm~\ref{alg:SMB2} with $\eta=\frac{1}{3}$, $\varepsilon=0.02$ and $T=3,\!000,\!000$.

\subsubsection{Results}



%Figure~\ref{fig:workload} depicts the work done at each time by the three users by Algorithm~\ref{alg:SMB2} (blue lines) and Proportional Greedy Algorithm~\ref{alg:PropGreedy} (green lines) in a randomly sampled load input sequence. Proportional Greedy is an algorithm that computes an optimal $1$-allocation and in each time ensures that each user gets an allocation proportional to her SLA. See Algorithm~\ref{alg:PropGreedy} in Appendix. Empirically, we observe that the work done by the users in Algorithm~\ref{alg:SMB2} tends to converge to their proportional share in each period. For example, in period $P_2=[500,\!000,\,1,\!000,\!000)$, users $1$ and $2$ do work approximately equal to $\frac{\beta(1)}{\beta(1)+\beta(2)} = 0.4$ and $\frac{\beta(2)}{\beta(1)+\beta(2)} = 0.6$, respectively.
%
%\begin{figure}[h!]
%	\centering
%	\begin{minipage}[b]{0.72\linewidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/work_user_0}
%%		\caption{default}
%%		\label{fig:exp1}
%	\end{minipage}\\
%	%	\hspace{0.5cm}
%	\begin{minipage}[b]{0.72\linewidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/work_user_1}
%%		\caption{default}
%%		\label{fig:exp2}
%	\end{minipage}\\
%	%	\hspace{0.5cm}
%	\begin{minipage}[b]{0.72\linewidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/work_user_2}
%%		\caption{default}
%%		\label{fig:exp3}
%	\end{minipage}
%	\caption{Work done by Algorithm~\ref{alg:SMB2} and Proportional Greedy in one random input. We can observe the change of behavior at time $t=1,\!500,\!000$.}
%	\label{fig:workload}
%\end{figure}
%
%%% old

%\textbf{Work maximization.} In Figure~\ref{fig:char3users} we present the log base 10 of the difference between the overall optimal work done by Proportional Greedy and Algorithm~\ref{alg:SMB2} in blue line. Additionally, in red color, we present the log base 10 of the difference between the overall work done by Algorithm~\ref{alg:SMB2} and the optimal work done by $(1-\varepsilon)$-allocations. For completeness, we present the function $\log_{10}(\varepsilon T)$ in green line as an upper bound. We observe that Algorithm~\ref{alg:SMB2} does significantly more work than the best $(1-\varepsilon)$-allocations. In average, the work done by Algorithm~\ref{alg:SMB2} surpasses the work done by $(1-\varepsilon)$-allocations by $0.7\%$. On the other hand, we observe an average difference of $0.01\%$ between the work done by Proportional Greedy and Algorithm~\ref{alg:SMB2}. Moreover, the difference between the work done by Proportional Greedy and Algorithm~\ref{alg:SMB2} is significantly below the theoretical guarantee. Indeed, Theorem~\ref{thm:mainextension} implies that $\log_{10}(\work_{\text{offline}} - \work_{\text{alg}}) \leq  \log (\mathcal{O}(\varepsilon^{-2}\log 1/\varepsilon + \varepsilon T ))$ and we see from the graph that the log-difference of both values is at most $\log_{10}(\varepsilon T)$. Running a simple regression we obtain that $\work_{\text{offline}} - \work_{\text{alg}} \approx \frac{1}{1000} T$.

%% old

\textbf{Work maximization.} In Figure~\ref{fig:char3users} we present the cumulative work difference between PG and Algorithm~\ref{alg:SMB2} (solid blue line with star), restPG and Algorithm~\ref{alg:SMB2} (red dashed line with triangle), PO and Algorithm~\ref{alg:SMB2} (solid magenta line), Static and Algorithm~\ref{alg:SMB2} (solid green line with small circle) and OWM and Algorithm~\ref{alg:SMB2} (solid cyan line with large circle). Intuitively, one positive unit of difference implies the corresponding algorithm is ahead of Algorithm~\ref{alg:SMB2} by one unit of time.

% ATH: I'm removing most of the explicit numbers here; not sure they add much.
First, we consider the comparison to online algorithms  Static, PO and OWM.  Algorithm~\ref{alg:SMB2} outperforms Static significantly, by roughly $700,\!000$ units of time. During the first half of the experiment PO shows good performance, but in the second half of the experiment (when the load distribution changes), Algorithm~\ref{alg:SMB2} outperforms PO. %by $17,\!000$ units of time by the end of the experiment.
This shows that Algorithm~\ref{alg:SMB2} can adapt to changing input sequences that PO cannot adapt to. Finally, OWM surpasses Algorithm~\ref{alg:SMB2} during the whole experiment, with a performance similar to PG; %By the end of the experiment, the difference of work is roughly $9,\!500$ units.
this is an expected result since OWM is work maximizing.

With respect to offline algorithms, PG outperforms Algorithm~\ref{alg:SMB2} by roughly $10,\!000$ time units. On the other hand, Algorithm~\ref{alg:SMB2} surpasses restPG by approximately $20,\!000$ units. This shows that Algorithm~\ref{alg:SMB2} indeed performs better than the offline optimum with a slightly reduced amount of resources, as guaranteed by the theoretical results.
%
\begin{figure}[h!]
	\centering
		\centering
	\includegraphics[width=0.75\linewidth]{figures/Char3users_log.png}
	\caption{Difference between algorithms' work. Alg is short for Algorithm~\ref{alg:SMB2}. Observe that the differences ``OPT - Alg'' ``and ``OWM - Alg'' slightly overlap.}
	\label{fig:char3users}
\end{figure}

\textbf{SLA satisfaction.} Among online algorithms, Static and PO satisfy SLA restrictions by design, but as seen earlier they are not competitive in terms of work maximization. We focus on the comparison between OWM and Algorithm~\ref{alg:SMB2} as far as SLA satisfaction is concerned. Although OWM performs extremely well in work maximization, this comes at a significant price in SLA satisfaction. In Figure~\ref{fig:work} we depict empirically this behavior by plotting the instantaneous work done by users $2$ and $3$ by OWM and Algorithm~\ref{alg:SMB2} during period $P_1$. We empirically observe that Algorithm~\ref{alg:SMB2} approximately satisfies user $3$'s SLA,  but OWM does not allocate the user any resources. Such an extreme behavior arises because OWM is geared towards work maximization rather than SLA satisfaction.
%
%During the first half of the experiment, the data is given in such a way that in each period one of the active user demands a large load in one time while the other active user demands her load step by step. This poses an issue to OWM since this online method will tend to assign all the resource to the user with a large load. Once this user has finished, OWM will shift away resource to the next set of active users. For instance, in period $P_1$, user $2$ demands at time $t=1$ a load of roughly $\frac{T}{6}\cdot \frac{\beta(2)}{\beta(2)+\beta(3)} = 187,\!500 $ units so she becomes the only active user at that moment . OWM will allocate to her the whole resource for  $\frac{T}{6}\cdot \frac{\beta(2)}{\beta(2)+\beta(3)}$ time steps. On the other hand, user $3$, which also demands resource in that period, will not receive any allocation until user $2$ has finished $\frac{T}{6}\cdot \frac{\beta(2)}{\beta(2)+\beta(3)}$ later.
%
\begin{figure}[h!]
	\centering
%	\begin{minipage}[l]{0.72\linewidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/work_user_onl_0}
%	\end{minipage}\\
%	\hspace{0.5cm}
	\begin{minipage}[l]{0.7\linewidth}
		\includegraphics[width=\textwidth]{figures/work_user_onl_1}
	\end{minipage}\\
	\begin{minipage}[l]{0.7\linewidth}
	\includegraphics[width=\textwidth]{figures/work_user_onl_2}
\end{minipage}\\
	\caption{Instantaneous work for user $2$ and $3$ during period $P_1$. User $3$ does not receive any allocation in OWM until user $2$ finishes all of their work.}
	\label{fig:work}
\end{figure}

\textbf{Queue lengths.} In Figure~\ref{fig:queuessquared} we present the $2$-norm of queues induced by Algorithm~\ref{alg:SMB2} (solid blue), Static (solid magenta with star), PO (solid cyan with large circle) and OWM (solid black with triangle). Once again, we can interpret one unit of norm as one unit of latency. Experimentally, we observe that Static shows the worst performance with a final $2$-norm of $524,\!000$ units. Algorithm~\ref{alg:SMB2} ends with a $2$-norm of $10,\!000$ units, PO with $26,\!970$ units, and OWM with $381$ units. As remarked above, even though OWM induces very small queues, this comes at the cost of not satisfying SLA requirements. % we remark that Algorithm~\ref{alg:SMB2} always reserves $\varepsilon/3$ units to any inactive users. Therefore, since in each period only $2$ users are active, Algorithm~\ref{alg:SMB2} loses approximately $\frac{\varepsilon}{3}\cdot T = 20,\!000$ units that could be potentially used with a finer implementation of Algorithm~\ref{alg:SMB2}.
%
\begin{figure}[h!]
		\centering
	\includegraphics[width=0.75\linewidth]{figures/Queues_squared}
	\caption{$2$-norm of queues.}
	\label{fig:queuessquared}
\end{figure}


{\textbf{Summary.} Among all online algorithms, Algorithm~\ref{alg:SMB2} is able to best balance work maximization and SLA satisfaction. In particular, Algorithm~\ref{alg:SMB2} is only slightly worse in terms of work maximization compared to OWM; this is expected since Algorithm~\ref{alg:SMB2} always reserves a small fraction of the resource for each user, regardless of activity. Furthermore, our results show that the actual total work done by Algorithm~\ref{alg:SMB2} is much better than the theoretical guarantee of Theorem~\ref{thm:mainextension}, as it substantially outperforms $(1-\varepsilon)$OPT (restPG). Finally, we observe small queues throughout the entire horizon, which is key for maintaining reasonable latencies.}


%\subsection{Lower Bound}

%In our second numerical experiment, we test work maximization against an adversarial input load. For the experiment, we consider two users with equal SLAs $\beta(1)= \beta(2)= 0.5$. We also set $\eta=0.1$ and $\varepsilon= \frac{1}{T^{1/5}}$. In this experiment we will measure $\work_{\text{offline}} - \work_{\text{alg}}$, where $\work_{\text{offline}}$ is the optimal work offline given by $1$-allocations and $\work_{\text{alg}}$ is the work done by Algorithm~\ref{alg:SMB1}.

%In this experiment, the load is adversarially constructed following the ideas in the proof of Theorem~\ref{thm:GeneralLB}. Throughout all the experiment, we enforce that both users' allocations are close to their SLAs. This is easily achieved by keeping them most of the time active. The experiment is divided into \emph{phases}. At the beginning of each phase only one user has a nonempty queue, say of length $Q$. We will transfer this active user's queue to the other one by loading $(0,1)$ or $(1,0)$ accordingly. This will take roughly $2Q$ time steps. At the end of the phase, the initial inactive user end ups with a queue of length approximately $Q+\frac{1}{2}$ and a new phase start. Since we are loading $(0,1)$ or $(1,0)$ at all time, the optimal offline work is $\work_{\text{offline}} = T$.

%We run the experiment for $T=10,000,000$ units of time. We make samples every $250,000$ units of time. In the left-hand side of Figure~\ref{fig:workcomparison} we plot the difference $\work_{\text{offline}} - \work_{\text{alg}} = T - \work_{\text{alg}}$ in blue, the curve $\sqrt{T}$ in red and the curve $T^{4/5}$ in green. As stated in Theorem~\ref{thm:GeneralLB} our algorithm has a loss at least $\sqrt{T}$ and as stated in Corollary~\ref{cor:UpperboundAlg} is at most $T^{4/5}$. In the right-hand side of Figure~\ref{fig:workcomparison} we plot the ratio $\work_{\text{alg}}/\sqrt{T}$ in red and the ration $\work_{\text{alg}}/{T^{4/5}}$. In this case, we observe that $T-\work_{\text{alg}}$ grows faster than $\sqrt{T}$ but not as fast as $T^{4/5}$.

%\begin{figure}[ht]
%	\centering
%	\begin{minipage}[b]{0.5\linewidth}
%		\centering
%	\includegraphics[width=\linewidth]{figures/work_comparison}
%	\end{minipage}\hfil
%	%	\hspace{0.5cm}
%	\begin{minipage}[b]{0.5\linewidth}
%		\centering
%	\includegraphics[width=\linewidth]{figures/work_comparison_ratio}
%	\end{minipage}
%	\caption{Work comparison.}
%	\label{fig:workcomparison}
%\end{figure}



\subsection{Experiment with Real Data}

%\subsubsection{Description of the experiments}~

We next describe the results of our computational study using real world data. For these experiments, we obtained CPU traces of a production service on Azure, Microsoft's public cloud. The data consists of demand traces of six different users over a time window of approximately ten days.


To show Algorithm~\ref{alg:SMB2}'s robustness with respect to (short-term) real data, we also consider the following measurement:
\begin{itemize}
%	\item \textbf{Work maximization.} We compare the overall work done by Algorithm~\ref{alg:SMB2} and the cumulative optimal work done by $1$-allocations and the cumulative optimal work done by $(1-\varepsilon)$-allocations. In order to compare Algorihtm~\ref{alg:SMB2} against online algorithms, we implemented an online version of Algorithm~\ref{alg:PropGreedy} (see Algorithm~\ref{alg:OnlProp} below). We decided not to display any work comparisons against the Static SLA Policy (every user gets her SLA) since Algorithm~\ref{alg:SMB2} surpassed the static policy with ease in terms of work maximization. In this experiment we expect that Algorithm~\ref{alg:SMB2} is  surpassed by the work done by the optimal $1$-allocations. Now, since there are few time steps, it is clear that Algorithm~\ref{alg:SMB2} will surpass the work done by $(1-\varepsilon)$-allocations as in the previous experiments. However, numerical experiments still show that Algorithm~\ref{alg:SMB2} performs well in practice.
%	
\item \textbf{Instantaneous SLA.} We focus on a modified SLA satisfaction criterion because of the relatively short horizon (about $14,000$ minutes); %, which is much shorter than the theoretical requirement to ensure SLA satisfaction (see Theorem~\ref{thm:SLAextension}).
we assess Algorithm~\ref{alg:SMB2}'s performance in the following way. For a user $i$ and any time $t$, we compare the cumulative work done by user $i$ in Algorithm~\ref{alg:SMB2} during a time window $[t,t+\tau)$ versus the cumulative work done by the same user $i$ under a Static SLA Policy during the time window $[t,t+\tau)$. In order to have a meaningful comparison, at time $t$, we run the Static SLA Policy with the queues of Algorithm~\ref{alg:SMB2} at time $t$. The motivating question is, \emph{what happens if at time $t$ and the next $\tau$ time steps we run the static policy instead of Algorithm~\ref{alg:SMB2}?} For this experiment, we used $\tau = 500$ minutes.% Our experiment suggests that Algorithm~\ref{alg:SMB2} ensures SLA under this metric most of the time for small time windows even though we do not present any theoretical guarantee. For our experiments, we used $\tau =500$ minutes.
	
	%
%	
%	\item \textbf{Queue lengths.} We compare the 2-norm of queues generated by the three following \emph{online algorithm}: Algorithm~\ref{alg:SMB2}, Static SLA Policy and Proportional Online. The reason to focus only on these algorithms is to obtain some insight about the queue lengths of different methods that solely possess limited information of the system. As in the previous experiment, we aim to measure the variance of the queues at each time for each of the algorithms and determine empirically whose algorithms show higher latency. We expect to surpass the performance of the Static SLA Policy due to the lack of adaptivity of the latter method and outdo the Proportional Online Algorithm.

\end{itemize}

The data set consists of demand traces of six users of exactly $14,\!628$ minutes (approximately ten days). Each user is assigned their normalized average workload as SLA. (Since the data is proprietary, we cannot disclose actual SLAs.) For the purpose of the experiment, we run Algorithm~\ref{alg:SMB2} with parameters $\varepsilon=0.01$ and $\eta = \frac{1}{3}$.



\subsubsection{Results}

%\textbf{Work maximization.} In Figure~\ref{fig:MS_work_users_ratio}, we present the three following ratios for each time $t$: cumulative work done until time $t$ by $1$-allocations and Algorithm~\ref{alg:SMB2}; $(1-\varepsilon)$-allocations and Algorithm~\ref{alg:SMB2}; and Proportional Online and Algorithm~\ref{alg:SMB2}. A ratio below $1$ means that Algorithm~\ref{alg:SMB2} outperforms the respective algorithm and a ratio greater than one means the opposite. Of course, compared to optimal $1$-allocations, the ratio always results at least $1$. However, from the data, we can observe that the optimal work done is just an average of $0.12\%$ greater than the work done by Algorithm~\ref{alg:SMB2} with a standard deviation of $0.4\%$. We can also observe empirically that Algorithm~\ref{alg:SMB2} is outperformed by the optimal work done by $(1-\varepsilon)$-allocations by an average of $0.003\%$. This is mostly due to the first 2000 minutes (see the graph). In this time period, an offline solution can adapt instantaneously surpassing the work done by Algorithm~\ref{alg:SMB2}. Compared to Proportional Online, we notice from the data that Algorithm~\ref{alg:SMB2} surpasses Proportional Online by approximately $0.2\%$ in cumulative work done. Comparison against Static SLA Policy is not shown here, but in average Algorithm~\ref{alg:SMB2} surpasses the Static SLA Policy by an average of $2\%$ and standard deviation of $1\%$.
%
%\begin{figure}[h!]
%	\centering
%	\includegraphics[width=0.75\linewidth]{figures/MS_work_users_ratio}
%	\caption{Ratio of cumulative works. Here Alg is a short for Algorithm~\ref{alg:SMB2}, OPT for optimal $1$-allocations, $(1-\varepsilon)$OPT for optimal $(1-\varepsilon)$-allocations and OnlineProp for Proportional Online.}
%	\label{fig:MS_work_users_ratio}
%\end{figure}
%
%
%Now, the ratio of Figure~\ref{fig:MS_work_users_ratio} becomes significant in the long-term since in the early stage, say before $2,\!000$ minutes, no significant amount of work has been done by any algorithm hence any fluctuation influence greatly the ratio. For this reason we depict in Figure~\ref{fig:MS_work_users_diff} the difference of the works done by the aforementioned algorithms. Here, one positive unit means one unit of lateness for Algorithm~\ref{alg:SMB2} and one negative unit means one unit of advantage for Algorithm~\ref{alg:SMB2}. Compared to the optimal $1$-allocations, we can notice an average lateness of $4.85$ units of time and increasing by the end of the term. Against the best $(1-\varepsilon)$-allocations the situation reverses. In early stages we observe an advantage from the offline algorithm, mostly due to its full-knowledge of the state of the system. However, since the offline algorithm's resource is slightly reduced, Algorithm~\ref{alg:SMB2} outperforms it in the long-term with an average of $4.9$ units of time over the entire period. Compared against Proportional Online, the circumstances are positive for Algorithm~\ref{alg:SMB2} by surpassing Proportional Online most of the time with an average of $11.2$ units of time. For completeness, Algorithm~\ref{alg:SMB2} outperforms Static SLA Policy by an average of $87.3$ units of time over the entire period and a maximum of $171$ units of time.


\textbf{Work maximization.} We depict in Figure~\ref{fig:MS_work_users_diff} the following differences: cumulative work done until time $t$ by optimal $1$-allocations (PG) and Algorithm~\ref{alg:SMB2}, $(1-\varepsilon)$-allocations (restPG) and Algorithm~\ref{alg:SMB2}, PO and Algorithm~\ref{alg:SMB2}, Static and Algorithm~\ref{alg:SMB2}, and OWM and Algorithm~\ref{alg:SMB2}. In a similar fashion to the previous experiment, one positive unit can be interpreted as Algorithm~\ref{alg:SMB2} being one unit (minute) of work behind, and one negative unit means Algorithm~\ref{alg:SMB2} is ahead by a minute.

We observe that Algorithm~\ref{alg:SMB2} outperforms all online benchmarks. Against Static, the final difference is $105$ units, with a maximum difference of $167$ units. Against PO the final difference is $25$ units with a maximum difference of $37$. Finally, against OWM, the final difference is $20$ with a maximum difference of $21$. Surprisingly, for this data set Algorithm~\ref{alg:SMB2} is able to surpass even OWM.

Regarding the offline algorithms, PG surpasses Algorithm~\ref{alg:SMB2} during the whole experiment as expected, with a final difference of $14$ units. On the other hand, Algorithm~\ref{alg:SMB2} outperforms restPG by $26$ units by the end of the experiment.
\begin{figure}[h!]
	\centering
	\includegraphics[width=0.75\linewidth]{figures/MS_work_users_diff}
	\caption{Difference of cumulative works.}
	\label{fig:MS_work_users_diff}
\end{figure}


\textbf{Instantaneous SLA.} In Table~\ref{tab:MS_diff_SLA} we report statistics on the differences between the cumulative work done in time windows $[t,t+\tau)$  by Static and Algorithm~\ref{alg:SMB2} for each user. For each $t$ and each user $i$, the exact formula is $r_i(t)={\sum_{r=t}^{t+\tau -1} w_r'(i)}-{\sum_{r=t}^{t+\tau -1} w_r(i)}$, where $w_r(i)$ is the work done by user $i$ under Algorithm~\ref{alg:SMB2} and $w_r'(i)$ is the work done by user $i$ with Static (with queues at $t$ given by Algorithm~\ref{alg:SMB2}). The table shows the min, max, average and standard deviation of $\{  r_i(t)\}_t$ when $\tau=500$ minutes. A positive unit means Algorithm~\ref{alg:SMB2} is outperformed by Static during $[t,t+\tau)$ under the same initial conditions by one unit of time. In general, we observe that all users show negative empirical average difference.  This result empirically suggests that Algorithm~\ref{alg:SMB2} ensures approximate SLA satisfaction, even for small time windows. For instance, user $3$ occasionally has a high difference (46.4 units), mostly due to times $t$ where Algorithm~\ref{alg:SMB2} allocates the user a small amount of resource but a huge load is incoming during the window $[t,t+\tau)$. The experiment tells us that averaging out these ``bad'' times ensures good performance under the SLA criterion. Furthermore, we tested values of $\tau=60$, $500$ and $1000$ minutes; larger windows improve the results, with lower maximum and average values.
%
%
\begin{table}
	\caption{Statistics for the difference between the cumulative works of our algorithm and static over time windows $[t,t+\tau)$. For each user $i$ we present the min, max, average, and standard deviation over the sequence of differences $\{ r_i(t) \}_{t}$.}
	\label{tab:MS_diff_SLA}
	
	\centering
	\begin{tabular}{|l|l|l|l|l|}
		\hline
		User   & min    & max  & mean  & std  \\
		\hline
		User 1 & -31.1  & 21.7 & -4.6  & 13.8 \\
		User 2 & -122.3 & 46.9 & -31.2 & 49.2 \\
		User 3 & -90.8  & 46.4 & -7.2  & 29.5 \\
		User 4 & -49.7  & 18.5 & -0.8  & 12.9 \\
		User 5 & -42.6  & 22.6 & -5.85 & 14.0 \\
		User 6 & -21.9  & 14.9 & -0.6  & 6.4 \\
		\hline
	\end{tabular}
\end{table}

\textbf{Queue lengths.} In Figure~\ref{fig:MS_Queues_squared} we present the $2$-norms of queues given by the online benchmark algorithms and Algorithm~\ref{alg:SMB2}. As usual, we can interpret one unit as the respective algorithm's latency, that is, lateness with respect to the overall users' demand. Compared against the online algorithms, we empirically observe the superiority of Algorithm~\ref{alg:SMB2}, as it has the smallest latency most of the time. Algorithm~\ref{alg:SMB2} ends with a $2$-norm of roughly 44 units, average length of 22 and a maximum length of 92. PO ends with a $2$-norm of approximately 68, average length of 32 and a maximum length of 126. OWM ends with a $2$-norm of 68, average of 32 and maximum of 113. Finally, Static shows the worst behavior, with a final $2$-norm of $103$, average of $91$ and maximum of $231$. For this data set, Algorithm~\ref{alg:SMB2} shows a remarkable performance, considering particularly that Algorithm~\ref{alg:SMB2} always reserves $\varepsilon/N$ resource for each user.

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.75\linewidth]{figures/MS_Queues_squared}
	\caption{$2$-norm of queues.}
	\label{fig:MS_Queues_squared}
\end{figure}

{\textbf{Summary.} Algorithm \ref{alg:SMB2} performs very well in terms of work maximization compared to all other online algorithms, and exceeds the theoretical guarantees. Furthermore, SLA requirements are typically satisfied, even when measured over relatively short time windows. Finally, as in the previous experiment, the algorithm maintains small queues compared to other online algorithms.
}% ATH: I am personally not a fan of so much recapping and summarizing, because this paper is already quite long. 








==> version arxiv/Extension.tex <==
\subsection{Extension to Proportionality and Over-commitment}\label{sec:Extension}

In the previous subsections, we have introduced the first version of the multiplicative weights algorithm. We explained how we deduced our algorithm using mirror descent and proved its theoretical guarantees. Even though Algorithm~\ref{alg:SMB1} guarantees individual SLA satisfaction, this simple policy can lead to undesirable results that do not respect the ratio between allocations. If one user has an SLA twice the size of another, it would be reasonable for the former to expect allocations at least twice as big as the latter's if both are consistently busy. Likewise, the second user would expect allocations no less than half of the first user's. In other words, both users should expect shares that respect the ratio between their SLAs.

To illustrate this unsatisfactory behavior in Algorithm~\ref{alg:SMB1}, we run it with three users having SLAs $\beta(1)=0.5$, $\beta(2)=0.3$ and $\beta(3)=0.2$. We set $\eta\leq 1/3$ and $\varepsilon\leq 1/10$. For simplicity, the initial allocation will be uniform. In our example, user $1$ is always idle. User $2$ consistently demands $1$ unit of resource. User $3$ begins idle and remains so until user $2$'s allocation reaches $1-\varepsilon$. This takes roughly $\frac{1}{\eta \varepsilon}$ time steps; call this time $t_0$. Starting at time $t_0$, user $3$ demands unit loads every time step for the rest of the horizon. Initially, the allocations are uniformly $1/3$ for everyone. Between time $1$ and $t_0$, user $2$'s allocation increases until it hits $1-\varepsilon$, since they are the only active user. After $t_0$, user $3$ becomes active, and has an allocation below their SLA. Therefore, the algorithm redistributes allocation from user $2$ to $3$ until user $3$'s allocation hits $0.2$. After this, allocations remain stable at approximately $h_t(1)= \frac{\varepsilon}{3}$, $h_t(2)= 0.8- \frac{\varepsilon}{3}$ and $h_t(3)=0.2$. User $2$ receives about $4$ times the allocation of user $3$ if $\varepsilon$ is small enough. However, a better allocation for user $2$ and $3$ is $\frac{\beta(2)}{\beta(2)+\beta(3)} = \frac{3}{5}$ and $\frac{\beta(3)}{\beta(2) + \beta(3)} = \frac{2}{5}$ respectively. These allocations reflect the ratio $\frac{\beta(2)}{\beta(3)}$ between active users.

Given this, we propose a slight modification of Algorithm~\ref{alg:SMB1}, shown in Algorithm~\ref{alg:SMB2}. As before, the plan is always to benefit active users. However, this time, we boost active users slightly more if they fall behind their ``proportional SLA'' among active users. Intuitively, if there are $n<N$ active users for a long period of time, the allocation of these active users should converge to their proportional share.
%
\begin{center}
	\begin{algorithm}[H]
		\KwIn{Parameters $0<\varepsilon\leq \frac{1}{10}, 0  <\eta < \frac{1}{3} $.}
		%		\KwData{this text}
		%	\KwResult{how to write algorithm with \LaTeX2e }
		Initialization: $\h_1$ any allocation over $\Delta_\varepsilon$ and $\lambda= \frac{\varepsilon^2}{8 N}$. \\
		\For{$t=1,\ldots,T$}
		{
			Set allocation $\h_t$.\\
			Read active and inactive users $A_t$ and $B_t$. $A_t^1=\left\{ i \in A_t : h_t(i)< (1-\varepsilon)\frac{\beta(i)}{\sum_{j\in A_t} \beta(j)} \right\}$, $A_t^2= A_t\setminus A_t^1$. \\
			Set gain function $g_t(i)=\begin{cases}
			1 + \lambda & i \in A_t^1\\
			1  & i\in A_t^2\\
			0  & i \in B_t
			\end{cases}$.\\
			Update allocation:
			$\widehat{h}_{t+1}(i)  = h_t(i)e^{\eta g_t(i)}, \forall i $ and $\h_{t+1} = \pi_{\Delta_\varepsilon}(\widehat{h}_{t+1})$
		}
		%\Return $S_k$
		\caption{Extended Multiplicative Weight Update Algorithm} \label{alg:SMB2}
	\end{algorithm}
\end{center}

For technical reasons, the set $A_t^1$, the active users with allocation below their proportional share among active users at time $t$, has to be defined as $\left\{ i \in A_t : h_t(i)< (1-\varepsilon)\frac{\beta(i)}{\sum_{j\in A_t} \beta(j)} \right\}$. The reason behind this choice is to ensure that if $A_t^1\neq \emptyset$ and the resource is nearly fully utilized, i.e., $\sum_{i\in A_t} h_t(i)\geq 1-\varepsilon$, then there is a different active user $j\neq i$ from which we can move allocation to $i$. This is fundamental in the proof of Theorem~\ref{thm:SLAextension} below.

In terms of work maximization and SLA satisfaction, Algorithm~\ref{alg:SMB2} provides exactly the same guarantees as Algorithm~\ref{alg:SMB1}.

\begin{theorem}\label{thm:mainextension}
	Given loads $L_1,\ldots,L_T$, for any $\varepsilon>0$ and $\eta >0$ such that $\varepsilon \leq 1/10$, Algorithm \ref{alg:SMB2} guarantees
	\[
	\work_{\h_1^*,\ldots,\h_t^*} - \work_{\text{alg},t} \leq 8\frac{N}{\varepsilon^2 \eta} \ln(N/\varepsilon),
	\]
for any time $1\leq t\leq T$, where $\h_1^*,\ldots,\h_T^*$ is an optimal offline sequence of $(1-4 \varepsilon )$-allocations and $\work_{\text{alg},t}=\sum_{i}\sum_{\tau=1}^t w_{\tau}(i)$ is the overall work done by Algorithm~\ref{alg:SMB2} until time $t$.
\end{theorem}

The proof of Theorem~\ref{thm:mainextension} is exactly the same as the proof of Theorem~\ref{thm:main1}. To see this, observe that the proof of Theorem~\ref{thm:main1} only uses the fact that the allocations of \emph{every} active user get a multiplicative boost whenever the usage is below $1-\varepsilon$. The last statement is true since Lemma~\ref{lem:monotonicity} also holds in this case.
%

For SLA satisfaction, we have the following stronger statement.
%
\begin{theorem}\label{thm:SLAextension}
	Let $0< \varepsilon\leq 1/10$, $0< \eta \leq 1/3$, $\lambda = \frac{\varepsilon^2}{8N}$ and $\tilde{p}=32 \frac{N^2}{\varepsilon^3 \eta} \ln (N/\varepsilon)$. Take any SLAs $\beta(1),\ldots,\beta(N)$ such that $\frac{\beta(i)}{\sum_k \beta(k)} \geq \frac{e^{\eta(1+\lambda)}}{1-\varepsilon} \frac{\varepsilon}{N}$. Then, for any user $i$ and time $t$, if we take $\h_1',\ldots,\h_T'$ to be the allocations such that $ h_t'(i)=\left(1-2\varepsilon\right) \frac{\beta(i)}{\sum_k \beta(k)}$, the work done by Algorithm \ref{alg:SMB1} for user $i$ satisfies
	\[
	\sum_{\tau=1}^{t+\tilde{p}} w_\tau(i) \geq \sum_{\tau = 1 }^t w_\tau'(i),
	\]
where $\w_t'$ is the work done by the allocations $\h_1',\ldots,\h_T'$. Moreover $\sum_{\tau=1}^t w_\tau(i) \geq \sum_{\tau=1}^t w_\tau'(i) - \frac{\beta(i)}{\sum_k \beta(k)}\tilde{p}$.
\end{theorem}
%
The proof of this result is similar to the proof of Theorem~\ref{thm:main2}. A subtle difference is that the analogue of Lemma~\ref{lem:monotonicity2} holds if we add the hypothesis $\sum_{i\in A_t} h_t(i) > 1-\varepsilon$. We skip the proof for brevity.
%
\begin{lemma}\label{lem:monotonicity3}
	Assume $\varepsilon\leq \frac{1}{10}$, $\eta \leq \frac{1}{3}$ and $\frac{\beta(i)}{\sum_k \beta(k)} \geq \frac{e^{\eta(1+\lambda)}}{1-\varepsilon} \frac{\varepsilon}{N}$ for all users. In Algorithm~\ref{alg:SMB2}, if $\sum_{k\in A_t} h_t(k)> 1- \varepsilon$ then for any $i\in A_t^1$ we have $h_{t+1}(i) \geq (1+c') h_t(i)$, where $c'= \frac{\varepsilon \eta \lambda}{2N}$.
\end{lemma}

Lemma~\ref{lem:monotonicity} and \ref{lem:monotonicity3} ensure that any active user gets a multiplicative boost of at least $(1+c')$. Therefore, any user that is active $\widetilde{p}$ consecutive times will have an allocation of at least $(1-2\varepsilon) \frac{\beta(i)}{\sum_k \beta(k)}$. Then, by following the same inductive proof of Theorem~\ref{thm:main2}, we obtain Theorem~\ref{thm:SLAextension}.

If the resource is not over-committed, $\sum_k\beta (k)\leq 1$, this result implies that Algorithm~\ref{alg:SMB2} ensures for each user $i$ an amount of work comparable with $\frac{\beta(i)}{\sum_k \beta(k)} \geq \beta(i)$; that is, we obtain the standard SLA satisfaction guarantee.
%
In the over-commitment regime, $\sum_{i=1}^N \beta(i)> 1$, we do retain some performance guarantees.  The update according to almost-normalized SLAs in Algorithm~\ref{alg:SMB2} still works and Theorem~\ref{thm:mainextension}'s work maximization guarantee still applies, as its proof does not rely on the SLAs. On the other hand, Theorem~\ref{thm:SLAextension} states that individually, each user does work comparable to their normalized SLA. If the level of over-commitment is not large, each user is still guaranteed service ``almost'' at their SLA; for example, if the resource is over-committed by $10\%$, each user receives service comparable to $1.1^{-1} \approx 91\%$ of their SLA.
%{\color{red} overcommitment or over-commitment?} % ATH: I prefer "over-commitment"

Another interesting byproduct of the work maximization guarantee is the following result.
\begin{corollary}
Under the assumptions of Theorem~\ref{thm:main2}, %let $L_1,\ldots,L_T$ be any sequence of loads. 
suppose there is a time $1\leq \tau\leq T$ with $\sum_{t=1}^\tau \sum_{i} w_\tau'(i)= \sum_{t=1}^\tau \sum_{i} L_t(i)$; i.e.\ the optimal offline $(1-4 \varepsilon)$-allocation is able to finish all work up until $\tau$. Then, the sum of queue lengths at time $\tau$ induced by Algorithm \ref{alg:SMB2} is at most $8\frac{N}{\varepsilon^2 \eta} \ln(N/\varepsilon)$. %ATH: Please verify if this phrasing is correct.
In particular, at time $\tau$ each user's queue length is at most this value. 
\end{corollary}

In practical settings, it is commonplace to assume an arrival rate is lower than the work processing rate. In stochastic settings, stationary states cannot be achieved without this assumption; see, e.g.,\ \cite{tassiulas1990stability}. In our context, this can be reinterpreted as having times within the operating horizon where the optimal offline solution is able to finish all work arriving up until that time. At these particular times, the corollary guarantees that Algorithm \ref{alg:SMB2}'s queue lengths are constant. In other words, the algorithm does not starve individual users to achieve work maximization and keeps their queues short, an appealing property in cloud systems. %it ensures a relatively good amount of SLA per user (depending of level of commitment) and has constant queue-length whenever the optimal offline solution is able to finish its work.}


==> version arxiv/Introduction.tex <==


\section{Introduction}

%% begin Alejandro's version

Cloud computing has motivated renewed interest in resource allocation, manifested in new consumption models (e.g., AWS spot pricing), as well as the design of resource-sharing platforms \citep{hindman2011mesos,vavilapalli2013apache}. These platforms need to support a heterogenous set of users, also called tenants, that share the same physical computing resource, e.g., CPU, memory, I/O bandwidth. Providers such as Amazon, Microsoft and Google offer cloud services with the goal of benefiting from economies of scale. However, the inefficient use of resources -- over-provisioning on the one hand or congestion on the other -- could result in a low return on investment or in loss of customer goodwill, respectively. Hence, resource allocation algorithms are key for efficiently utilizing cloud resources.

%% end Alejandro's version

%%% begin older version

%Cloud computing has brought renewed interest in resource allocation, manifested in new consumption models (e.g., AWS spot-pricing), as well as the design of resource-sharing platforms \citep{vavilapalli2013apache,hindman2011mesos}. These platforms need to support multiple and heterogenous set of users (tenants) that \emph{share} the same physical compute resources (e.g., CPU, memory, I/O bandwidth). Providers such as Amazon, Microsoft, Google etc.~offer cloud services with the goal of benefiting from the economy of scale. However, inefficient use of resources -- over-provisioning on the one hand or congestion on the other hand -- might result in low ROI or detrimental business impact, respectively. Hence, resource allocation \emph{algorithms} are key for efficiently utilizing cloud resources.
%provide multi-tenant services that share the same resources (CPU, memory, network bandwidth) on the same hardware across multiple tenants/users.

%%% end older version


%% Alejandro's version

To ensure quality of service, cloud offerings often come with a \emph{service level agreement} (SLA) between the provider and the users. An SLA specifies the amount of resource the user is entitled to consume. Perhaps the most common example is renting a virtual machine (VM) that guarantees an explicit amount of CPU, memory, etc. Naturally, VMs that guarantee more resources are more expensive. In this context, a simple allocation policy is to assign each user the resources specified by their SLAs. However, such an allocation can be wasteful, as users may not need the resource at all times. In principle, a dynamic allocation of resources can increase the total efficiency of the system. However, allocating resources dynamically without carefully accounting for SLAs can lead to user dissatisfaction.


Recent scheduling proposals address these challenges through work-maximizing yet fair schedulers \citep{zaharia2010delay,ghodsi2011dominant}. However, such schedulers do not have explicit SLA guarantees. On the other hand, other works focus on enforcing SLAs \citep{rayon,morpheus,grandl2016altruistic}, but do not explicitly optimize the use of extra resources.

%% end Alejandro's version

%%% begin older version
%To ensure quality of service, cloud offering often come with a service level agreement (SLA) between the provider and the users. These SLAs specify the amount of resources the user is entitled to consume. Perhaps the most common example is renting a VM, which comes with an explicit amount of CPU, memory, etc. Naturally, VMs that guarantee more resources are priced higher. In this context, one simple allocation policy is to assign each user the resources specified by the SLAs. However, such allocation can be wasteful, as some users may not need resource at any given time. In principle, a dynamic allocation of resources can increase the total efficiency of the system. However, allocating resources dynamically without carefully accounting for the SLA can lead to user dissatisfaction.

%Recent scheduling proposals address the above challenges through work-conserving yet fair schedulers \citep{zaharia2010delay,ghodsi2011dominant}. However, such schedulers do not have explicit SLA guarantees. On the other hand, other works focus on enforcing SLAs \citep{rayon,morpheus,grandl2016altruistic}, but do not explicitly optimize the use of extra resources.
%%% end older version


%while ensuring that each user gets the same performance as if it received the same amount of resources as specified in the SLA.
%Nowadays, companies provide multi-tenant cloud computing services. Multi-tenancy is essential to make the service cost-effective by economy of scale. However, statically reserving resources for a tenant is not cost effective.

%When workloads from multiple tenants contend for shared resources, tenant's performance may be affected by the demand of other tenants.

%In this paper, we study the problem of how to effectively share a resource (CPU) in a multi-tenant system in the most fair way.


%%% begin Alejandro's version

Our goal in this work is to understand the fundamental tradeoff between high utilization of resources and SLA satisfaction of individual users. In particular, we design algorithms that guarantee \emph{both} near optimal utilization as well as the satisfaction of individual SLAs, simultaneously. To that end, we formulate a basic model for online dynamic resource allocation. We focus on a single divisible resource, such as CPU or I/O bandwidth, that has to be shared among multiple users. Each user also has an SLA that specifies the fraction of the resource it expects to obtain. The actual demand of the user is in general time-varying, and may exceed the fraction specified in the SLA. As in many real systems, the demand is not known in advance, but rather arrives in an online manner. Arriving demand is either processed or queued up, depending on the resource availability. In many real-world scenarios, it is difficult to measure the actual demand size (see, e.g., \cite{SQLVM}). Accordingly, we assume that the system (and the underlying algorithm) receives only a simple \emph{binary feedback} per user at any given time: whether the user queue is empty (the user's work arriving so far has been completed), or not. This is a plausible assumption in many systems, because one can observe workload activity, yet anticipating how much of the resource a job will require is more difficult. Additionally, it also models settings where demands are not known in advance.

While online dynamic resource allocation problems have been studied in different contexts and communities (see Section \ref{sec:related} for an overview), our work aims to address the novel aspects arising in the cloud computing paradigm, particularly the presence of SLAs, the highly limited feedback about the state of the system, and a desired robustness over arbitrary input sequences. For the algorithm design itself, we pay close attention to practicality; our approach involves fairly simple computations that can be implemented with minimal overhead of space or time. Our algorithm achieves nearly optimal utilization of the resource, as well as approximately satisfying the SLA of each individual user. We see two main use-cases for the algorithm:
%
\begin{itemize}
\item In enterprise settings (``private cloud''), different applications or organizations share the same infrastructure. These often have SLAs, but providers would still like to maximize the ROI by maximizing utilization \citep{mercury}.
\item In public clouds, users buy VMs, which are offered at different ``sizes'' (which is practically the SLA). In addition, the service providers offer ``best-effort'' alternatives, such as Azure Batch (MS) or Spot instances (AWS). In our model, these services can be modeled by giving an SLA of zero. Here, satisfying the VM SLAs and achieving high utilization are both important; indeed, the provider is paid for the best-effort workloads only if it completes these jobs. Our work can be viewed as a principled way to accommodate such services, and even give VMs better service than expected, an important consideration as public cloud offerings gradually become commoditized.
\end{itemize}
%%% end Alejandro's version


%%% begin older version
%Our goal in this work is to design algorithms that guarantee \emph{both} high utilization, while satisfying individual SLAs. To that end, we formulate a basic model for online dynamic resource allocation. We focus on a single divisible resource such as CPU or I/O bandwidth that has to be shared among many users. Each user also has his own SLA that specifies the fraction of the resource that it expects to obtain. The actual demand of the user is in general time varying, and may exceed the fraction specified in the SLA. As in many real systems, the demand is not known in advance, but rather arrives in an online manner. The demand is either processed or queued up depending on the resource availability. In real scenarios, it is very hard to measure the actual demand size (see, e.g., \citep{SQLVM}). Accordingly, we assume that the system (and underlying algorithm) receives only a simple binary feedback per user at any given time: whether the user queue is empty (i.e., all the demand of the user has been satisfied so far), or not. This is a plausible assumption in many systems, because one can observe workload activity, yet it is much harder to anticipate how much resources would be consumed.


%While online dynamic resource allocation problems have been studied in different contexts and communities (see Section~\ref{sec:related} for an overview), our work aims to address the novel aspects of this problem which arise in the cloud computing paradigm: presence of SLAs that have to be respected; highly limited feedback about the state of the system, and robustness over arbitrary input sequences. For the algorithm design itself, we pay close attention to practicality: our algorithm involve fairly simple computations that can be implemented with minimal overhead of space or time. We give simple and efficient algorithms that achieve nearly optimal efficient utilization of the resource, as well as approximately satisfying the SLA of each individual user. We see two main use-cases for these algorithms:



%\begin{itemize}
%\item In enterprise settings (“private-cloud”), different applications/organizations share the same infrastructure. These often have SLAs, but providers still would like to maximize the ROI by maximizing utilization \citep{mercury}.
%\item In public clouds, users buy VMs, which are offered at different “sizes” (which is practically the SLA). Here, high utilization is also important. Consequently, cloud providers offer “best-effort” alternatives, such as Azure Batch (MS), Spot instances (AWS). Our work can be viewed as a principled way to accommodate such services, and even give VMs better service than expected, which could be meaningful as basic cloud services are gradually becoming a commodity.
%\end{itemize}
%%% end older version

\subsection{The Model}

We consider the problem of having multiple tenants or users sharing a single resource, such as CPU, I/O or networking bandwidth. For simplicity, we assume that the total resource capacity is normalized to $1$. We have $N$ users sharing the resource, a finite but possibly unknown discrete time horizon indexed $t=1,\ldots, T$, and an underlying queuing system. For each user $i$, we are also given an expected share of resource $\beta(i)\geq 0$ satisfying $\sum_{i=1}^N \beta(i)\leq 1$. The input is an online sequence of workloads $L_1,\ldots,L_T\in \R_+^N$, where $L_t(i)\geq 0$ corresponds to $i$'s workload  arising at time $t$. The system maintains a queue $Q_t(i)$, denoting $i$'s remaining work at time $t$. In our model, the decision maker does \emph{not} have direct access to the values of the queues or the workloads. This allows us to consider settings where the job sizes are not known in advance and minimal information is available about the underlying system, a regular occurrence in many cloud settings. At time $t$, the following happens:
%
\begin{enumerate}
\item \textbf{Feedback:} The decision maker observes which queues are non-empty (the set of users $i$ with $Q_t(i)>0$, the \emph{active} users), and which are empty ($ Q_t(i) = 0 $, the \emph{inactive} users). %For users with non-empty queues, the decision maker does not receive any feedback regarding the length of the queues apart from the fact that it is non-empty.
	
\item \textbf{Decision:} The decision maker updates user resource allocations $h_{t}(i)$, satisfying $\sum_i h_t(i)\leq 1$.
	
\item \textbf{Update:} The load $L_t(i)$ for each $i$ arrives and each user processes as much of the work from the queue plus the arriving workload as possible. The work completed by user $i$ in step $t$ is
	$$w_t(i):=\min\{h_t(i), L_t(i)+Q_t(i)\}.$$
	The queues at the end of the time step are updated accordingly,
	\[Q_{t+1}(i) = \max\{0, L_t(i) + Q_t(i) - h_t(i)\}.\]
\end{enumerate}
%
%
We assess the performance of any algorithm based on two measures.
\begin{enumerate}
	\item \textbf{Work Maximization.} The algorithm should maximize the total work completed over all users, and thus utilize the resource as much as possible.
	\item \textbf{SLA Satisfaction.} The algorithm should (approximately) satisfy the SLAs in the following manner. The work completed by user $i$ up to any time $1\leq t \leq T$ should be no less than the work completed for this user up to $t$ if it were given a constant $ \beta(i) $ fraction  of the resource over the whole horizon.
\end{enumerate}
%
Achieving either of the criteria on their own is straightforward. A greedy strategy that takes away resources from an idle user and gives them to any user whose queue is non-empty is approximately work-maximizing (see Appendix~\ref{sec:localgreedy} for details). On the other hand, to satisfy the SLAs, we give each user a \emph{static} assignment of $h_t(i):=\beta(i)$ for all $t$. Naturally, the two criteria compete with each other; the following examples illustrate why these simple algorithms do not satisfy both simultaneously.




%%% begin older version
%We consider the problem of having multiple tenants/users sharing a single resource, for example, the CPU or I/O or networking bandwidth. For simplicity, we assume that the total resource capacity is normalized to $1$. The model is set as follows. We have $N$ users sharing the resource, a finite, but unknown, discrete time horizon numbered $t=1,\ldots, T$ and an underlying queuing system. For each user $i$, we are also given an expected share of resource $\beta(i)\geq 0$ such that $\sum_{i=1}^n\beta(i)\leq 1$. The input is an online sequence of workloads $L_1,\ldots,L_T\in \R_+^N$, where $L_t(i)\geq 0$ corresponds the workload of user $i$ at time $t$ that are hidden from the decision maker. Additionally, the system maintains a queue $Q_t(i)$ at each time $t$ for each user $i$ denoting the remaining work still to be done at time $t$. In our model, the decision maker does \emph{not} have any access to the values of the queues or the loads. This allows us to model settings where the job sizes are not known in advance and minimal information is available about the underlying system, a regular occurrence in many cloud applications. At time $t$, the following happens:

%\begin{enumerate}
%\item \textbf{Feedback:} The decision maker receives the feedback which queues are empty at time $t$, i.e., the set of users $i$ such that $Q_t(i)=0$. %For users with non-empty queues, the decision maker does not receive any feedback regarding the length of the queues apart from the fact that it is non-empty.

%\item \textbf{Decision:} The decision maker updates the allocation $h_{t}(i)$ for the next time step for each user $i$ such that $\sum_i h_t(i)\leq 1$.


%\item \textbf{Update:} The load $L_t(i)$ for user $i$ arrives and each user tries to complete as much workload from the arriving workload $L_t(i)$ plus the queued up work not done in previous steps $Q_{t}(i)$. Thus work done for user $i$ in this step is $$w_t(i):=\min\{h_t(i), L_t(i)+Q_t(i)\}.$$  The queues at the end of the time step are updated accordingly: for each user $i$, $Q_{t+1}(i) = \max\{0, L_t(i) + Q_t(i) - h_t(i)\}$.
%\end{enumerate}





%We aim to measure the performance of any algorithm based on two measures.
%\begin{enumerate}
%\item \textbf{Work Conservation.} The algorithm should aim to utilize as much resources as possible and maximize the total work done over all users.
%\item \textbf{SLA Satisfaction.} Secondly, the algorithms should aim to (approximately) satisfy the SLAs for each user $i$. Thus the work done up to any time $1\leq t \leq T$ for any user $i$ should be the at least the work done for this user if it were given $\beta_i$ fraction of the resource for all time steps till $t$.
%\end{enumerate}


%Achieving each of the criteria on their own is quite straightforward. A greedy strategy that only takes away resources from an user whose queue is empty and gives it to any user whose queue is non-empty is (approximately) work-conserving, see appendix \ref{sec:localgreedy}. It is also straightforward to satisfy the SLAs by giving each user a static assignment of $h_t(i):=\beta(i)$ for all $t$. Naturally, the above two criteria compete with each other. The following input sequences illustrate why these simple algorithms don't satisfy both these criteria.
%%% end older version


\begin{figure}[h!]
	
	\centering
	
	\includegraphics[width=1.01\linewidth]{figures/graph-1}
	\caption{Example of loads and work for 3 users. The blue dashed lines show each user's workload. The green areas represent the work done by the users. The red dashed lines depict SLAs.}
	\label{fig:graph}
\end{figure}

\begin{example}
	We have a shared system with three users and corresponding SLAs $\beta(1)= 0.5, \beta(2)=0.2$ and $\beta(3)=0.3$. Loads are defined by
	{\small\[
		L_t(1)=\begin{cases}
		1 & t=1,\ldots,T/3,2T/3+1,\ldots,T\\
		0 & t=T/3+1,\ldots,2T/3
		\end{cases}, \text{ and} \quad L_t(2)=L_t(3)= 1- L_t(1).
		\]}
	We assume that $T$ is divisible by $3$. In Figure~\ref{fig:graph} we show the three users' loads in blue dashed lines and the corresponding SLAs in dotted red lines. The static solution given by the SLAs, i.e.\ $h_t(i)=\beta(i)$ for all $t$, ensures a total of $5T/6$ work done. However, the dynamic policy shown in the green line, given by
	{\small
		\begin{center}
			\begin{tabular}{|c|c|c|c|}
				\hline
				$t$ & $[0,T/3]$ & $[T/3+1,2T/3]$ & $[2T/3+1,T]$\\
				\hline
				$h_t(1)$ & $1$    & $0$  & $0.5$\\
				\hline
				$h_t(2)$ & $0$    & $0.4$  & $0.2$\\
				\hline
				$h_t(3)$ & $0$    & $0.6$  & $0.3$\\
				\hline
			\end{tabular}
		\end{center}
	}
\noindent ensures $T$ work is done (the green area). Moreover, it also ensures SLA satisfaction at all times. An alternative policy is
	{\small
		\begin{center}
			\begin{tabular}{|c|c|c|c|}
				\hline
				$t$ & $[0,T/3]$ & $[T/3+1,2T/3]$ & $[2T/3+1,T]$\\
				\hline
				$h_t(1)$ & $1$    & $0$  & $0$\\
				\hline
				$h_t(2)$ & $0$    & $1$  & $0$\\
				\hline
				$h_t(3)$ & $0$    & $0$  & $1$\\
				\hline
			\end{tabular}\\
		\end{center}
	}
\noindent which is also work maximizing. However, it does not ensure SLA satisfaction. Indeed, this policy does not satisfy user $3$'s SLA at any time in $(T/3,2T/3]$.
\end{example}

We remark that achieving both criteria is relatively simple if we allow the decision maker to observe demand or even the queue length. This can be achieved by first allocating to each user as much of the resource as necessary up to their SLA, and then distributing the remaining resource arbitrarily among users with additional demand. % If the queue length is visible, the algorithm can let the first period pass without allocating anything to any user, so that each queue stores the first period's demand. From the second period onward, the algorithm acts as if demand exactly matches the queue lengths. It first allocates to each user with non-empty queue as much resource as necessary up to their SLA, and the remaining capacity is distributed arbitrarily among users with queue length longer than their initial allocation. This strategy clearly satisfies SLA requirements, and is work maximizing up to an additive constant of $1$ (because of the idle first period). The same algorithm and analysis apply if the decision maker is allowed to observe the demand.
The versatility of our setting stems from the limited feedback in the form of binary information about idle and busy users. In our cloud computing context, full demand information or even visible queue lengths are unrealistic assumptions.

%\begin{example}[Maximizing utilization may imply SLA violation]
%Consider two users with equal SLAs, $\beta(1)=\beta(2) = 0.5$. Consider the loads $L_t(1) = L_t(2) = 1$ for $t=1,\ldots,T/2$ and $0$ for $t=T/2+1,\ldots,T$. Clearly, the policy $h_t(1) = 1$ for $t=1,\ldots,T/2$ and $h_t(2)=1$ for $t=T/2+1,\ldots,T$ is work-maximizing. However, this policy does not satisfy SLA satisfaction. Indeed, until time $T/2$ user $2$ has done $0$ work while the fixed policy $\beta(2)$ has done $T/2$ work.
%\end{example}



%\begin{example}[Focusing solely on the SLA may imply poor utilization]
%Consider again two users with the same SLAs, $\beta(1)=\beta(2)=0.5$. Let $L_t(1)=0.2$ and  $L_t(2)=0.8$ for all $t\leq T$. The static allocation $h_t(1)=h_t(2)=0.5$ for all $t$ satisfies the SLAs at all time but is inefficient. At any time $t$, the total work completed under this allocation is $0.7 t$; the alternative static allocation $ h_t'(1) = 0.2 $, $ h_t'(2) = 0.8 $ maximizes utilization, completing $t$ units of work at time $t$, and satisfies users' SLAs. %Moreover, no user should be unhappy since at all time they are completing their work.
%\end{example}



%The model is set as follows: The decision maker distributes the processor among $N$ users. For simplicity, we assume that the total capacity of the processor is normalized to $1$. The $N$ users load tasks in the processor sequentially. At time $t$, the decision maker set an allocation $\h_t(i)$ for each of the $N$ users such that $\sum_i \h_t(i)\leq 1$. At the same time, each user tries to load her tasks $L_t(i)$ plus any previous work not done in the past into the processor. The decision maker receives as \emph{feedback} the real usage of the processor $\w_t \leq \h_t$. All the incomplete work is saved in a queue that we denote as $Q_t$, and this work is added up to future loads. The decision maker does not get any information about the queues. Finally, the decision maker updates $\h_{t+1}$ for the next time.



\subsection{Our Results and Contributions}


We design a simple and efficient online algorithm that achieves approximate work maximization as well as approximate SLA satisfaction even in the limited feedback model that we consider. For work maximization, we analyze the performance by comparing our algorithm to the \emph{optimal offline dynamic allocation} that knows all the data up front. In contrast, our online algorithm receives limited  feedback even in an online setting.  Thus, our aim  is to minimize the quantity $$\work_{\h_1^*,\ldots,\h_T^*} -\work_{\text{alg}} = \sum_{t=1}^T \sum_i w_t^*(i)  - \sum_{t=1}^T \sum_i w_t(i),$$
where $\work_{{\h}_1^*,\ldots,{\h}_T^*}$ is the optimal offline work done by dynamic allocations $\h_1^*,\ldots,\h_T^*$ , $\w_t^*= (w_t^*(1),\ldots, w_t^*(N)) $ is the work done at time $t$ by these allocations, and $\work_{\text{alg}}$ is the work done by the algorithm with allocations $\h_1,\ldots,\h_T$ and work $\w_t= (w_t(1),\ldots, w_t(N))$ at time $t$. The objective of the decision maker is to \emph{minimize} this quantity by constructing a sequence of good allocations that approach the best allocations in hindsight. Note that our benchmark is \emph{dynamic}, rather than the more common \emph{static} offline optimum usually considered in regret minimization \citep{arora2012multiplicative,hazan2016introduction,shalev2012online}. Similarly, for SLA satisfaction, our benchmark is the total work done for a user if they were given $\beta(i)$ resources for each time $1\leq t\leq T$. We give a bi-criteria online algorithm that achieves nearly the same performance as the benchmarks if the resources for the latter are slightly more constrained than that of the algorithm.
%{\color{red}
Algorithm~\ref{alg:SMB1}, which we formally describe in Section \ref{sec:algorithm}, follows a multiplicative weight approach. The idea is to boost the allocations of active users by a factor greater than $1$, with more emphasis on users with current allocation below their SLA. This intuition translates into a simple update that ensures high utilization of the resource and SLA satisfaction; formally:
%}

\begin{theorem}\label{thm:main} For any input parameter $0<\varepsilon\leq \frac{1}{10}$, SLAs $\beta=(\beta(1),\ldots,\beta(N))$ satisfying $\beta(i) \geq  2\frac{\varepsilon}{N}$, and online loads $L_1,\ldots,L_T\in \R_{\geq 0}^N$, Algorithm~\ref{alg:SMB1} achieves the following guarantees:
	%
	\begin{enumerate}
		\item \textbf{Approximate Work Maximization.}  Let $\h_1^*,\ldots,\h_T^*\in [0,1]^N$ be an optimal offline sequence of allocations such that $\sum_i h_t^*(i)=1$ for all $1\leq t\leq T$. Then
		\[
		\textstyle	\work_{\text{alg}} \geq  (1-\varepsilon) \work_{\h_1^*,\ldots,\h_T^*} -  \mathcal{O} \left({N {\varepsilon^{-2}\log(N/\varepsilon) }}\right).
		\]
		
		
		\item \textbf{Approximate SLA Satisfaction.} There exists $\tilde{p} = \tilde{p}(N,\varepsilon) =\mathcal{O} \left( N^2 \varepsilon^{-3}  \log (N/\varepsilon)  \right)$ such that for any user $i$ and time $t$, if we take $\h_1',\ldots,\h_T'\in [0,1]^N$ to be any sequence of allocations with $h_t'(i)\leq \beta(i)$, then
		\[
		%\sum_{\tau=1}^{t} w_\tau(i) \geq \sum_{\tau = 1 }^{t-s} w_\tau'(i)\geq \sum_{\tau = 1 }^{t} w_\tau'(i) -\beta_i\cdot s
			\sum_{\tau=1}^{t} w_\tau(i) \geq \left(1-2\varepsilon\right) \sum_{\tau = 1 }^{t}  w_\tau'(i) -\beta(i) \tilde{p} ,
		\]
		where $\w_t'$ is the work performed by the allocations $\h_1',\ldots,\h_T'$.
	\end{enumerate}
\end{theorem}

The first part of Theorem~\ref{thm:main} asserts that if $T$ is known for the system, we can achieve $\work_{\text{offline}}-\work_{\text{alg}}\leq \mathcal{O}(T^{2/3}\log T)$ with $\varepsilon= \Theta\left(\frac{N^{1/3}}{T^{1/3}}\right)$. %ATH: Since we now include the dependence on N below, I think it makes more sense to just include it here too.
However, this choice of $\varepsilon$ is suboptimal for SLA satisfaction. We can achieve an improved bound for SLA satisfaction (when $t=T$) by picking $\varepsilon= \Theta\left(\frac{N^{1/3}}{T^{1/4}}\right)$. If $T$ is unknown, we can use a standard doubling trick, see for example \citep{shalev2012online}. Summarizing, we obtain the following result.
%
\begin{corollary}\label{cor:UpperboundAlg}
	For $\varepsilon= \Theta\left( \frac{N^{1/3}}{T^{1/4} }  \right)$, Algorithm~\ref{alg:SMB1}  guarantees
	$$\textstyle \work_{\h_1^*,\ldots,\h_T^*} - \work_{\text{alg}} \leq \mathcal{O}(N^{1/3} T^{3/4} + N^{1/3} T^{1/2} \log(N T) ) =\mathcal{O}(N^{1/3}T^{3/4}) ,$$
	where $\h_1^*,\ldots,\h_T^*$ are optimal offline dynamic allocations.
\end{corollary}	

%Ths bound is tight for Algorithm~\ref{alg:SMB1} up to a logarithmic factor. Indeed, Algorithm~\ref{alg:SMB1} has a canonical hard input: overload one user. We can show that if we constantly load $1$ unit of work to user $1$ and $0$ to the rest, then the cumulative loss will be at least $\Omega(T^{2/3})$.
As $T$ grows, Corollary~\ref{cor:UpperboundAlg} guarantees that the \emph{rate} of work done by our algorithm $\frac{\work_{\text{alg}}}{T}$,
approaches the rate of work done by the optimal dynamic solution $\frac{\work_{{\h}_1^*,\ldots,{\h}_T^*}}{T}$.
We emphasize again that this is a stronger guarantee using the much more powerful optimal dynamic solution as a benchmark, rather than the typical static allocation used in regret analysis for online algorithms. Such a guarantee can be obtained in our model because the incomplete work remains stored in the queues until we are able to finish it; this allows the algorithm to \emph{catch up} with the incomplete work. %ATH: Removing this last sentence, as the same thing is repeated below when Theorem 2 is actually stated. %In Theorem~\ref{thm:GeneralLB_main}, we give a general lower bound showing our result is nearly optimal.

The second result in Theorem~\ref{thm:main} states that the work done by any individual user is comparable to the work done by their promised SLA. In other words, the user's queue length is not much larger than it would be under a static SLA allocation. By using $\varepsilon= \Theta\left( \frac{N^{1/3}}{T^{1/4}} \right)$ we obtain the following result.
%
\begin{corollary}\label{cor:Queues}
	Let $\varepsilon= \Theta\left( \frac{N^{1/3}}{T^{1/4}}  \right) $. For a user $i$,  $Q_T(i) \leq Q_{T}'(i) + \mathcal{O}(NT^{3/4}\log (NT))$, where $Q_t$ is the queue given by Algorithm~\ref{alg:SMB1} and $Q_t'$ is the queue induced by any dynamic policy $\h_1',\ldots,\h_T'$ with $h_t'(i)\leq \beta(i)$.
\end{corollary}

We remark that we need to bound the SLAs away from $\frac{\varepsilon}{N}$; in Theorem~\ref{thm:main} we use the bound $\beta(i)\geq 2\frac{\varepsilon}{N}$. This condition is necessary in our analysis to guarantee that there is an over-provisioned ($h_t(i)>\beta(i)$) user from which we can move allocation to an under-provisioned user. See Theorem~\ref{thm:main2} for details and a more relaxed bound.

%
%ATH: Isn't this exactly what we say above?
%We can use \emph{latency} as an alternate measure of user satisfaction. Corollary~\ref{cor:Queues} states that the {latency} $Q_T(i)$ will not be much larger than the promised quality of service given by the SLA, even with our limited feedback.

Corollary~\ref{cor:UpperboundAlg}'s guarantee is near-optimal asymptotically in $T$ in terms of work maximization, as the following result shows. The proof of this result appears in Appendix~\ref{sec:Lower}.
%
\begin{theorem}\label{thm:GeneralLB_main}
	For any online deterministic algorithm $\mathcal{A}$ for our model, there is a sequence of online loads $L_1,\ldots,L_T$ such that $\work_{\h_1^*,\ldots,\h_T^*} - \work_\mathcal{A} = \Omega\left(\sqrt{T}\right)$, where $\h_1^*,\ldots,\h_T^*$ are optimal offline dynamic allocations.
\end{theorem}

%Observe that for a fixed $\varepsilon$, the algorithm is comparing itself to the benchmark that is slightly over-constrained and achieves nearly the same performance up to an additive term that is independent of the length of the sequence. We emphasize that in 1., the offline sequence $\h_1^*,\ldots,\h_T^*$ ignores the SLAs and solely maximizes throughput. We also remark that in 2, once the user has been chosen, the sequence $\h_1',\ldots,\h_T'$ can be arbitrary, and in particular, we can choose the fixed allocations $\h_t' = (1-\frac{\varepsilon^2}{2N})\beta(i)$.


%We emphasize in Theorem~\ref{thm:main}, the benchmark for work conservation is the optimal offline \emph{dynamic} policy. This is in contrast to regret-style analysis of online algorithms where, typically, the benchmark is the optimal offline \emph{static} policy.

%Our algorithm follows two different multiplicative weight strategies depending on the limited feedback received. If the users with empty queues are assigned more than a fraction $\varepsilon$ of the resource, the decision maker updates the allocations greedily by penalizing these users. On the other hand, if $ 1 - \varepsilon $ or more of the resource is assigned to users with non-zero queues, and thus most of the resource is being utilized, the decision maker redistributes the resource by penalizing those users assigned more than their corresponding SLAs. The penalizing rates are distinct in the two cases and are chosen appropriately. We show that this efficient heuristic strategy is enough to achieve approximate work maximization and SLA satisfaction.


Our algorithm follows a mirror descent approach \citep{ben2001lectures,hazan2016introduction}. Unable to see the lengths of the queues, a (naive) approach is to pretend that active users have gigantic queues. From this approach we extract a simple update rule that multiplicatively boosts active users; however, active users who are under their SLA are boosted slightly more than other active users. If inactive users are assigned more than $\varepsilon$ of the resource, where $\varepsilon$ is the algorithm parameter, active users ramp up their allocation in few iterations. In the opposite case, at least $1-\varepsilon$ of the resource is assigned to active users, and the slight boost to users below their SLA ensures a healthy re-balancing of the resource.  We show that this efficient heuristic strategy is enough to achieve approximate work maximization and SLA satisfaction. We remark that the mirror descent interpretation is only used to provide intuition for the algorithm, and our proofs follow a different path than the usual mirror descent analysis. Later, we detail a slight modification that enjoys the same theoretical guarantees as Algorithm~\ref{alg:SMB1} but in practice exhibits more desirable behavior (see Algorithm~\ref{alg:SMB2}). Intuitively, among active users, the modified algorithm tries to keep allocations proportional to their SLAs. This behavior is appealing; for example, a user $A$ with twice the SLA of another user $B$ would expect in practice to perform at least twice as much work. Similarly, user $B$ would expect to receive no less than half of user $A$'s allocation. This second algorithm exhibits another interesting feature; it can be applied to over-committed regimes with $\sum_{i=1}^N \beta (i) > 1$, remain work-maximizing, and satisfy a normalized version of SLA satisfaction (see Section~\ref{sec:Extension}).

%Indeed, in Theorem~\ref{thm:main1} and Theorem~\ref{thm:main2}, we show that the algorithm achieves a stronger guarantee than in Theorem~\ref{thm:main}. We show that the algorithm achieves the same guarantee as a slightly over-constrained offline dynamic policy up to an additive factor.

The analysis of the algorithm relies on a primal-dual fitting approach. For work maximization, we can write the offline dynamic optimal allocation as a solution to a linear program and then construct feasible dual solutions with objective value close to the algorithm's resource utilization. A crucial ingredient of the algorithm is the use of entropic projection on the \emph{truncated} simplex, which ensures every user gets at least a $\varepsilon/N$ fraction of the resource at all times. Intuitively, this means any user with a non-empty queue will recover their SLA requirement in a few steps.

%\paragraph{Experiments.}
We do an extensive analysis of our algorithm on synthetic data as well as real data obtained from CPU traces of a production service in Microsoft's cloud. We aim to quantify the performance of the algorithm on three objectives, (i) work maximization, (ii) SLA guarantee and (iii) queue behaviour. While our theoretical results give guarantees for these objectives, we show experimentally that the algorithm exceeds these guarantees. We benchmark the algorithm against natural online algorithms, such as a static allocation as given by the SLA guarantee, or the algorithm that aims to proportionally distribute the resource among active clients (according to their SLA). We also benchmark against offline algorithms that know all input data up front; our algorithm's performance on various measures is comparable to the offline algorithms.


% Our result is in bi-criteria form which trades off the performance of the algorithm with the allocations size. Specifically, we compare the performance of the allocations given by of our algorithm with the optimal offline allocations where the offline allocations must be of size at most $1-\mathcal{O}(\varepsilon)$.


This work is organized as follows. In Section \ref{sec:algorithm}, we present the preliminaries and the basic version of the multiplicative weight algorithm. Section \ref{sec:Analysis} contains the proof of Theorem \ref{thm:main} in the bi-criteria form. We split the proof into two parts: work maximization in Section \ref{sec:throughput} and SLA satisfaction in \ref{sec:SLAsat}. In Section \ref{sec:Extension}, we present the extension of our algorithm and its guarantees. Finally, in Section~\ref{sec:Numerical} we present numerical experiments that empirically validate our results, and conclude in Section \ref{sec:Conclusions}.



%In Appendix~\ref{sec:Lower}, we show a general lower bound for all online deterministic algorithms that allocate a divisible resource with the same feedback as our model. The lower bound shows that the guarantee for work maximization in Theorem~\ref{thm:main} is nearly tight for certain ranges of parameters.  %\ps{Is it alright the LB here?.}





==> version arxiv/lowerbound.tex <==
\section{Lower Bound}\label{sec:Lower}


\begin{theorem}\label{thm:GeneralLB}
	For any online deterministic algorithm $\mathcal{A}$ setting at each time $1$-allocations, with an underlying queuing system, and with the same limited feedback as Algorithm~\ref{alg:SMB1}, there exists a sequence of online loads $L_1,\ldots,L_T$ such that $\work_{\h_1^*,\ldots,\h_T^*} - \work_\mathcal{A} = \Omega\left(\sqrt{T}\right)$, where $\h_1^*,\ldots,\h_T^*$ are the optimal offline dynamic $1$-allocations.
\end{theorem}

\begin{proof}
	We consider the case with $N=2$ users, the general case reduces to $N=2$ by loading jobs only to two users. Let $\mathcal{A}$ be an online algorithm for allocating a divisible resource for $2$ users and with underlying queuing system and limited feedback. Without loss of generality, we can assume that the allocations sets by $\mathcal{A}$ always add up to $1$ at every time step.

	We will construct a sequence of loads $L_t = (L_t(1), L_t(2))$ that at every time will add up to $1$. This will ensure that the overall work done by the optimal offline dynamic policy will be $T$. On the other hand, we will show that this sequence of loads will lead to large queue length for at least one of the users.  The main ingredient is to use the fact the algorithm receives limited feedback about the state of the system, i.e., which users have empty queue. In particular, this implies that if there are two distinct set of load vectors $L_t$ and $L'_t$ for  some interval $t\in [r,s]$ such that the queues remain non-empty on both these sequences, then the resource allocation to the users in the two load sequences must be identical. 
	
	We will divide the time window $[1,T]$ into phases. Each phase will begin with a configuration of queues, say $Q= (Q(1), Q(2) )$, where one of the queues is empty and the other one nonempty. We set $q= Q(1)+Q(2)$ and we denote by $q_i$ the $q$ at phase $i$. We define $q_0 = 0$. We will prove that at the end of each phase $i\geq 1$, $q_{i+1}\geq q_i+\frac{1}{4}$ with all $q_{i+1}$ cumulated in one queue and the other queue empty.
	
	Initially, the algorithm has a fixed deterministic allocation $\h_1 = (h_1(1), h_1(2) )$. If $h_1(1)\leq h_1(2)$, then we load $L_1 =(0,1)$. Otherwise, we load $L_1 = (1,0)$. In any case, we have $q_1\geq \frac{1}{2}$ and all $q_1$ in one queue.
	
	Now, we will describe how the general phases work. For the sake of simplicity, we will describe the phase starting at time $t=1$. We have queue configuration $Q  =  ( Q(1), Q(2) ) $ with $q>0$. By the initial phase, we can assume $q\geq 1/2$. Moreover, we can assume that only one of the queues is nonempty, this point will be clear after we describe how the phase works and it is clearly true for phase $1$. Phase $i$ with $q=q_i$ will last at most $2q + 2$ time steps.
	
	Suppose that $Q(1)=0$ and $Q(2)>0$. If $h_1(1)=1$, then we load $L_1=(0,1)$ and the phase ends with $q$ increased by $1$ and user $1$'s queue empty. Therefore, we can assume $h_1(1)<1$. Our first load will be $L_1 =  (h_1(1)+\varepsilon, h_2(2)-\varepsilon) $ with $0<\varepsilon<\frac{1}{4}$ small enough and such that both queues are nonempty. The following loads will be $L_t=\h_t$, the allocation of $\mathcal{A}$ at time $t$. Observe that the first load will ensure that both users see nonempty queues until the end of the phase. Moreover, user $1$ always has exactly $\varepsilon$ remaining in her queue.
	
	\begin{itemize}
		\item If there is a time $\tau^\star \in [1, 2q+1]$ such that $h_{\tau^\star}(1)\geq 1/2$, then we change the load at time $\tau^\star$ for $L_{\tau^\star}' = (0,1)$. This will increment $q$ by at least $1/2-\varepsilon \geq 1/4$ and the phase ends. Observe that $Q_{\tau^\star+1}(1)=0$.
		
		\item We can assume now that for the loads $L_t=\h_t$ we always have $h_t(1)<1/2$ for all $t\in [2,2q+1]$. We change the loads to $L_t'=(1,0)$ until time $\tau^\star$ in which user $2$ empties her queue. Recall that the feedback of the algorithm is only the set of empty queues at every time step. Thus the behavior of $\mathcal{A}$ under $L_t$ and $L_t'$ will be the same until time $\tau^\star$. Now, we change load $L_{\tau^\star}$ by $L_{\tau^\star}' = ( 1 - h_{\tau^\star}(2) + Q_{\tau^\star}(2) -\varepsilon'  ,  h_{\tau^\star}(2) - Q_{\tau^\star}(2) + \varepsilon'  )$ with $0<\varepsilon'<1/4$ small enough. This will ensure that queue $2$ will be exactly $\varepsilon'$. Now, in an extra step, we load $L_{\tau^\star+1}=(1,0)$. Again, we have $q$ increased by at least $1/4$ and this ends the phase. Observe that $Q_{\tau^\star+2}(2)=0$.
	\end{itemize}

	The analysis is similar for $Q(1)>0$ and $Q(2)=0$. Observe that at the end of each phase, only one queue is nonempty and the other one is empty. In any case, we have the desired increment. With this, we can set the following recurrence, $
	q_0 = 0, \quad q_{i-1} + \frac{1}{4} \leq q_{i} \quad \forall i\geq 1$.	We deduce that $q_i \geq i/4$. Now, let $m$ be the number of phases. By construction, each phase last at most $2 q_i +2$. Then $T \leq \sum_{i=1}^m (2q_i +2) \leq 40 q_m^2$, where we have used $ 4q_m\geq4 q_i \geq i \geq 1$. From here we deduce that $q_m \geq \sqrt{T/40}$.
	
	Now, the work done by the algorithm and the unfulfilled work in the queues must add up the overall load. Then $q_m + \work_\mathcal{A} = T = \work_{\h_1^*,\ldots,\h_T^*}$	from which we obtain the result.
\end{proof} 

==> version arxiv/related.tex <==
\subsection{Related Work}\label{sec:related}


%%%%%% general literature

There has been growing interest in resource allocation problems arising from cloud computing applications, both from a practical as well as a theoretical standpoint \citep{grandl2016altruistic,hindman2011mesos,mercury,morpheus,rayon,SQLVM,vavilapalli2013apache,narasayya2015sharing,menache2015online}. The focus of many of these works has been to understand the trade-offs between efficiency and ensuring guarantees to individual users.


%%%%%% Stoch literature


%\modif{A large literature has been dedicated to stochastic arrivals with unknown but random demands, which have been closely studied for network bandwidth allocation and related problems.
%The assumption of stochastic arrivals is crucial to the analysis and results in this stream of literature~\citep{maguluri2012stochastic,maguluri2014heavy,maguluri2014scheduling, neely2008order}. Many of these models draw inspiration from queuing network models~\citep{tassiulas1990stability,tassiulas1993dynamic}, such as uplink and downstream scheduling in wireless network settings~\citep{neely2007optimal,neely2008order}. These results incorporate a network structure on the demands, describe the resulting queuing behavior, and characterize the stability region of the arrival processes. %; in contrast to our work, however, they rely crucially on stochastic arrival assumptions.
%In contrast, in our work we assume an adversarial input and very limited knowledge of the state of the system. Despite this difference, there are staggering parallels between the two approaches that worth mentioning for the interested readers. We design algorithms with rate of work $\frac{\work_{\text{alg} } }{T}$ approaching the optimal offline rate of work (Corollary~\ref{cor:UpperboundAlg}). Similar results hold for individual rate of work. This is comparable to the positive recurrence of the Markov process in many of these stochastic models and the notion of stabilization of the system~\citep{tassiulas1990stability, neely2007optimal} which in few words means bounded delay (queue length). Much of the stochastic literature assume complete knowledge of the arrival/systems statistics, including queue lengths. Nonetheless, there are fascinating works that limit the information obtained from the system in a similar fashion as we do (see~\cite{li2009energy, neely2007optimal,maguluri2014scheduling, shirani2010mimo}) but they do require the input to come from specific distributions to guarantee their results.
%}

On the more theoretical side, the cloud computing allocation problem has been modeled as a stochastic allocation problem \citep{maguluri2014heavy, maguluri2012stochastic, maguluri2014scheduling}. The underlying models draw inspiration from a large body of work on stochastic network control, originating from the seminal work of
\citet{tassiulas1990stability,tassiulas1993dynamic}, followed by additional related research, e.g., on uplink and downstream scheduling in wireless networks \citep{neely2007optimal,neely2008order}. The analytical results in these papers characterize the stability region of the arrival processes under certain stochastic assumptions (e.g., i.i.d.~processes), and suggest algorithms that achieve maximal throughput. The main distinction between these works and ours is that we assume an \emph{adversarial} input, i.e., we do not make stationary distributional assumptions on the input. Another difference is that our model centers on the notion of an SLA which is known to the algorithm. This allows us to address the over-commited case (see Algorithm~\ref{alg:SMB2}), which is especially relevant in cloud settings.

%a SLA guarantee and very limited knowledge of the state of the system.

Despite these modeling differences, there are some parallels worth mentioning. For example, we design algorithms with rate of work $\frac{\work_{\text{alg} } }{T}$ approaching the optimal offline rate of work; this translates to the average delay $\frac{1}{T}\sum_{t=1}^T \sum_{i=1}^N Q_t(i)$ converging to the optimal offline average delay. This result can be compared to the limiting behavior of the Markov process in many of the stochastic network models. For example, \cite{neely2008order} studies a system of $N$ users connecting to a server via ON/OFF channels. The paper presents an algorithm that ensures bounded average delay $\limsup_T \frac{1}{T} \E\left[ \sum_{t=1}^T \sum_{i=1}^N Q_{i}(t)  \right]$ for any input within the interior of the stability region; here $Q_i(t)$ is the $i$-th user's backlog (queue length) at time $t$. Much of the stochastic network literature assumes full knowledge of queue lengths, e.g.\ the LCQ policy in \citet{tassiulas1993dynamic}, although there are studies that limit the information available to the decision maker in a similar fashion to our model (see \citet{li2009energy, neely2007optimal,maguluri2014scheduling,shirani2010mimo}). %Nonetheless, the analysis of these models still requires stationary stochastic inputs satisfying additional conditions, as opposed to our adversarial framework.}

%%%%%%%%%%%%
%%%%%%%%%%%%
%This contrast of stationary/adversarial, queue length based feedback/binary feedback, positive recurrence/rate stability, would be interesting to the readers familiar with that literature
%%%%%%%%%%%%
%%%%%%%%%%%%

More broadly, the general problem of online resource allocation has been studied in both stochastic and adversarial settings; we refer the reader to the books \citep{albers2003online,borodin2005online,srikant2013communication} on the topic. Our work differs from the aforementioned lines of research by combining the three following elements already present in the literature. First, as mentioned above, we digress from the stochastic arrival model to the adversarial setting and worst-case analysis. This makes our algorithm robust against unpredictable users' demands. For instance, demands in the morning could be totally different from demands in the afternoon or the morning of the next day. We are able to provide a single strategy that adapts easily to any scenario. Second, we provide simple online algorithms that perform well even under \emph{limited feedback}, a typical situation in cloud systems in which we can only determine the utilization of a resource after it has been allocated. Finally, we consider SLA satisfaction as a measure of user contentment, and seek to satisfy it up to a small error.


%%%% Some extensions

There is now an extensive literature devoted to the pricing of cloud computing services. In \citep{macias2011genetic} the authors study a genetic model for generating a suitable pricing function in the cloud market. In \citep{gera2011learning}, pricing is studied via a revenue management formulation to address resource provisioning decisions. See also \citep{passacantando2016service,sharma2012pricing} for more pricing models. A closely related topic is fairness in resource allocation \citep{zaharia2010delay,ghodsi2011dominant}. Although we do not directly consider pricing, work maximization could be interpreted as a way to obtain extra revenue by allocating unused resources to active users.


More recently, there has been work considering over-commitment in the cloud \citep{cohen2019overcommitment,gordon2011ginkgo,dabbagh2015efficient}, that is, selling resources beyond server capacity. One of the objectives of over-commitment is to reduce the number of servers opened in order to minimize energy consumption. In our basic model, we do not assume over-commitment, yet our algorithm can still be applied to that setting (see Algorithm~\ref{alg:SMB2}). Specifically, we obtain a normalized version of SLA satisfaction in the over-commitment setting, where the guarantees depend on how much the system is over-committed (see Section~\ref{sec:Extension}).

%Work on cloud computing scheduling~\citep{}.
%The problem can be seen as an online optimization problem. Online convex optimization has been a growing area in recent years, , . In this setting, the decision maker chooses a point $\x_t$ and an adversary chooses a convex function $f_t(\x_t)$. The decision maker incurs in a loss $f_t(\x_t)$ and objective is to minimize the regret $\sum_t f_t(\x_t) - \sum_t f_t(\x^*)$, where $\x^*$ is the best decision in hindsight. Usually, the feedback is twofold. In the \emph{full information setting}, the feedback usually is the gradient or a subgradient of $f_t$ at $\x_t$. This information has proven to be enough to guarantee low-regret algorithms \citep{zinkevich2003online}. On the other hand, we have the \emph{bandit setting} in which the only feedback that the decision maker gets to see is the cost of the chosen arm. However, in the latter, the decision space is finite and this fact is strongly used to construct low-regret algorithms.

%In our case, $f_t(\h_t)=\sum_i \w_t(i)$ corresponds to the reward at time $t$. As a feedback we obtain $\w_t\leq \h_t$. Observe that $\w_t(i)=\min\{ L_t(i) + Q_t(i), \h_t(i)  \}$, therefore, the current reward $f_t$ depends on previous allocations and loads. However, the evaluation of these reward functions in the best allocations in hindsight is pointless: $f_{t+1}$ depends on $\h_t$ and $Q_t$ and not $\h_t^*$ (the optimal allocations). In this regard, and to the best of our knowledge, our contribution is the study of a new online optimization model with partial feedback that has a very natural application in CPU allocation.

%%%% Online Optimization literature

A fundamental tool in our design is \emph{mirror descent} algorithms \citep{ben2001lectures}. These first-order iterative algorithms have been widely used in optimization \citep{ben2001lectures}, online optimization and machine learning \citep{hazan2016introduction,mohri2018foundations,shalev2012online} to generate update policies under limited feedback. Similarly, multiplicative weights algorithms have been widely studied in optimization \citep{plotkin1995fast,arora2012multiplicative}, online convex optimization \citep{hazan2016introduction}, online competitive analysis \citep{buchbinder2009design} and learning theory \citep{freund1997decision,shalev2012online}. Our results bear some resemblance to regret analysis, where typically the benchmark is the optimal offline static policy \citep{shalev2012online,hazan2016introduction,abernethy2008optimal,bubeck2012regret,freund1997decision}; the use of a dynamic benchmark (as in our work) is scarcer in the literature, see e.g.\ \citet{hall2015online,mokhtari2016online,zinkevich2003online,zhang2017improved}.

